pytest-inline: An Inline Testing Tool for Python

We present pytest-inline, the first inline testing framework for Python. We recently proposed inline tests to make it easier to test individual program statements. But, there is no framework-level support for developers to write inline tests in Python. To fill this gap, we design and implement pytest-inline as a plugin for pytest, the most popular Python testing framework. Using pytest-inline, a developer can write an inline test by assigning test inputs to variables in a target statement and specifying the expected test output. Then, pytest-inline runs each inline test and fails if the target statement's output does not match the expected output. In this paper, we describe our design of pytest-inline, the testing features that it provides, and the intended use cases. Our evaluation on inline tests that we wrote for 80 target statements from 31 open-source Python projects shows that using pytest-inline incurs negligible overhead, at 0.012x. pytest-inline is integrated into the pytest-dev organization, and a video demo is at https://www.youtube.com/watch?v=pZgiAxR_uJg.

==> defs/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
  frame=tb,
}

\lstset{escapeinside={(*@}{@*)}}

\lstdefinelanguage{python-pretty}{
  language=Python,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
  sensitive=false,
  comment=[l]{\#},
  morecomment=[s]{/*}{*/},
  frame=tb,
}

\lstdefinelanguage{java-diff}
{
  language=java,
  numbers=left,
  numbersep=1.2pt,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  frame=lines,
  showstringspaces=false,
  morecomment=[f][\color{red!80!black}]-,         % deleted lines 
  morecomment=[f][\color{green!30!black}]+,       % added lines
}

\lstdefinelanguage{bash-pretty}
{
  language=bash,
  % numbers=left,
  % numbersep=1.2pt,
  basicstyle=\scriptsize\ttfamily,
  % numberstyle=\scriptsize,
  breaklines=true,
  % frame=lines,
  showstringspaces=false,
  morecomment=[f][\color{red!80!black}]-,         % deleted lines 
  morecomment=[f][\color{green!30!black}]+,       % added lines
}
%%%==========


==> defs/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> tables/data-combine-languages.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{NumTotalProjs}{68}
\DefMacro{NumTotalFiles}{100}
\DefMacro{NumTotalInlineTests}{152}
\DefMacro{NumTotalTestedStmts}{144}
\DefMacro{exp-total-proj-can-run-unit-tests}{21}
\DefMacro{exp-java-skipped-all}{30}
\DefMacro{exp-total-skipped-all}{47}
\DefMacro{exp-python-skipped-all}{17}


==> tables/data-exp-integrated-java.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-java-alibaba_fastjson-time-vanilla-dup1}{44.99}
\DefMacro{exp-java-alibaba_fastjson-time-unit-dup1}{44.86}
\DefMacro{exp-java-alibaba_fastjson-time-inline-dup1}{0.73}
\DefMacro{exp-java-alibaba_fastjson-time-unit-and-inline-dup1}{45.59}
\DefMacro{exp-java-alibaba_fastjson-num-vanilla-dup1}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-unit-dup1}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-inline-dup1}{2}
\DefMacro{exp-java-alibaba_fastjson-num-unit-and-inline-dup1}{5,024}
\DefMacro{exp-java-alibaba_fastjson-timept-vanilla-dup1}{0.009}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-dup1}{0.009}
\DefMacro{exp-java-alibaba_fastjson-timept-inline-dup1}{0.363}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-and-inline-dup1}{0.009}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-dup1}{-0.003}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-and-inline-dup1}{0.013}
\DefMacro{exp-java-alibaba_nacos-time-vanilla-dup1}{249.45}
\DefMacro{exp-java-alibaba_nacos-time-unit-dup1}{249.93}
\DefMacro{exp-java-alibaba_nacos-time-inline-dup1}{0.74}
\DefMacro{exp-java-alibaba_nacos-time-unit-and-inline-dup1}{250.67}
\DefMacro{exp-java-alibaba_nacos-num-vanilla-dup1}{971}
\DefMacro{exp-java-alibaba_nacos-num-unit-dup1}{971}
\DefMacro{exp-java-alibaba_nacos-num-inline-dup1}{1}
\DefMacro{exp-java-alibaba_nacos-num-unit-and-inline-dup1}{972}
\DefMacro{exp-java-alibaba_nacos-timept-vanilla-dup1}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-unit-dup1}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-inline-dup1}{0.745}
\DefMacro{exp-java-alibaba_nacos-timept-unit-and-inline-dup1}{0.258}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-dup1}{0.002}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-and-inline-dup1}{0.005}
\DefMacro{exp-java-apache_dubbo-time-vanilla-dup1}{678.86}
\DefMacro{exp-java-apache_dubbo-time-unit-dup1}{679.43}
\DefMacro{exp-java-apache_dubbo-time-inline-dup1}{0.82}
\DefMacro{exp-java-apache_dubbo-time-unit-and-inline-dup1}{680.26}
\DefMacro{exp-java-apache_dubbo-num-vanilla-dup1}{3,180}
\DefMacro{exp-java-apache_dubbo-num-unit-dup1}{3,180}
\DefMacro{exp-java-apache_dubbo-num-inline-dup1}{1}
\DefMacro{exp-java-apache_dubbo-num-unit-and-inline-dup1}{3,181}
\DefMacro{exp-java-apache_dubbo-timept-vanilla-dup1}{0.213}
\DefMacro{exp-java-apache_dubbo-timept-unit-dup1}{0.214}
\DefMacro{exp-java-apache_dubbo-timept-inline-dup1}{0.822}
\DefMacro{exp-java-apache_dubbo-timept-unit-and-inline-dup1}{0.214}
\DefMacro{exp-java-apache_dubbo-overhead-unit-dup1}{0.001}
\DefMacro{exp-java-apache_dubbo-overhead-unit-and-inline-dup1}{0.002}
\DefMacro{exp-java-apache_kafka-time-vanilla-dup1}{9.84}
\DefMacro{exp-java-apache_kafka-time-unit-dup1}{10.09}
\DefMacro{exp-java-apache_kafka-time-inline-dup1}{0.67}
\DefMacro{exp-java-apache_kafka-time-unit-and-inline-dup1}{10.76}
\DefMacro{exp-java-apache_kafka-num-vanilla-dup1}{221}
\DefMacro{exp-java-apache_kafka-num-unit-dup1}{221}
\DefMacro{exp-java-apache_kafka-num-inline-dup1}{1}
\DefMacro{exp-java-apache_kafka-num-unit-and-inline-dup1}{222}
\DefMacro{exp-java-apache_kafka-timept-vanilla-dup1}{0.045}
\DefMacro{exp-java-apache_kafka-timept-unit-dup1}{0.046}
\DefMacro{exp-java-apache_kafka-timept-inline-dup1}{0.670}
\DefMacro{exp-java-apache_kafka-timept-unit-and-inline-dup1}{0.048}
\DefMacro{exp-java-apache_kafka-overhead-unit-dup1}{0.026}
\DefMacro{exp-java-apache_kafka-overhead-unit-and-inline-dup1}{0.094}
\DefMacro{exp-java-apache_shardingsphere-time-vanilla-dup1}{5.03}
\DefMacro{exp-java-apache_shardingsphere-time-unit-dup1}{5.04}
\DefMacro{exp-java-apache_shardingsphere-time-inline-dup1}{0.71}
\DefMacro{exp-java-apache_shardingsphere-time-unit-and-inline-dup1}{5.75}
\DefMacro{exp-java-apache_shardingsphere-num-vanilla-dup1}{44}
\DefMacro{exp-java-apache_shardingsphere-num-unit-dup1}{44}
\DefMacro{exp-java-apache_shardingsphere-num-inline-dup1}{2}
\DefMacro{exp-java-apache_shardingsphere-num-unit-and-inline-dup1}{46}
\DefMacro{exp-java-apache_shardingsphere-timept-vanilla-dup1}{0.114}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-dup1}{0.115}
\DefMacro{exp-java-apache_shardingsphere-timept-inline-dup1}{0.355}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-and-inline-dup1}{0.125}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-dup1}{0.002}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-and-inline-dup1}{0.143}
\DefMacro{exp-java-jenkinsci_jenkins-time-vanilla-dup1}{4.67}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-dup1}{4.64}
\DefMacro{exp-java-jenkinsci_jenkins-time-inline-dup1}{0.65}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-and-inline-dup1}{5.29}
\DefMacro{exp-java-jenkinsci_jenkins-num-vanilla-dup1}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-dup1}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-inline-dup1}{2}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-and-inline-dup1}{34}
\DefMacro{exp-java-jenkinsci_jenkins-timept-vanilla-dup1}{0.146}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-dup1}{0.145}
\DefMacro{exp-java-jenkinsci_jenkins-timept-inline-dup1}{0.325}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-and-inline-dup1}{0.156}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-dup1}{-0.007}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-and-inline-dup1}{0.132}
\DefMacro{exp-java-skylot_jadx-time-vanilla-dup1}{66.57}
\DefMacro{exp-java-skylot_jadx-time-unit-dup1}{75.47}
\DefMacro{exp-java-skylot_jadx-time-inline-dup1}{0.74}
\DefMacro{exp-java-skylot_jadx-time-unit-and-inline-dup1}{76.21}
\DefMacro{exp-java-skylot_jadx-num-vanilla-dup1}{709}
\DefMacro{exp-java-skylot_jadx-num-unit-dup1}{709}
\DefMacro{exp-java-skylot_jadx-num-inline-dup1}{1}
\DefMacro{exp-java-skylot_jadx-num-unit-and-inline-dup1}{710}
\DefMacro{exp-java-skylot_jadx-timept-vanilla-dup1}{0.094}
\DefMacro{exp-java-skylot_jadx-timept-unit-dup1}{0.106}
\DefMacro{exp-java-skylot_jadx-timept-inline-dup1}{0.738}
\DefMacro{exp-java-skylot_jadx-timept-unit-and-inline-dup1}{0.107}
\DefMacro{exp-java-skylot_jadx-overhead-unit-dup1}{0.134}
\DefMacro{exp-java-skylot_jadx-overhead-unit-and-inline-dup1}{0.145}
\DefMacro{exp-java-time-vanilla-AVG-dup1}{151.34}
\DefMacro{exp-java-time-vanilla-SUM-dup1}{1,059.41}
\DefMacro{exp-java-time-vanilla-MAX-dup1}{678.86}
\DefMacro{exp-java-time-vanilla-MIN-dup1}{4.67}
\DefMacro{exp-java-time-vanilla-MEDIAN-dup1}{44.99}
\DefMacro{exp-java-time-vanilla-STDEV-dup1}{229.70}
\DefMacro{exp-java-time-vanilla-CNT-dup1}{7}
\DefMacro{exp-java-time-unit-AVG-dup1}{152.78}
\DefMacro{exp-java-time-unit-SUM-dup1}{1,069.47}
\DefMacro{exp-java-time-unit-MAX-dup1}{679.43}
\DefMacro{exp-java-time-unit-MIN-dup1}{4.64}
\DefMacro{exp-java-time-unit-MEDIAN-dup1}{44.86}
\DefMacro{exp-java-time-unit-STDEV-dup1}{229.46}
\DefMacro{exp-java-time-unit-CNT-dup1}{7}
\DefMacro{exp-java-time-inline-AVG-dup1}{0.72}
\DefMacro{exp-java-time-inline-SUM-dup1}{5.06}
\DefMacro{exp-java-time-inline-MAX-dup1}{0.82}
\DefMacro{exp-java-time-inline-MIN-dup1}{0.65}
\DefMacro{exp-java-time-inline-MEDIAN-dup1}{0.73}
\DefMacro{exp-java-time-inline-STDEV-dup1}{0.05}
\DefMacro{exp-java-time-inline-CNT-dup1}{7}
\DefMacro{exp-java-time-unit-and-inline-AVG-dup1}{153.50}
\DefMacro{exp-java-time-unit-and-inline-SUM-dup1}{1,074.53}
\DefMacro{exp-java-time-unit-and-inline-MAX-dup1}{680.26}
\DefMacro{exp-java-time-unit-and-inline-MIN-dup1}{5.29}
\DefMacro{exp-java-time-unit-and-inline-MEDIAN-dup1}{45.59}
\DefMacro{exp-java-time-unit-and-inline-STDEV-dup1}{229.50}
\DefMacro{exp-java-time-unit-and-inline-CNT-dup1}{7}
\DefMacro{exp-java-num-vanilla-AVG-dup1}{1,454.14}
\DefMacro{exp-java-num-vanilla-SUM-dup1}{10,179}
\DefMacro{exp-java-num-vanilla-MAX-dup1}{5,022}
\DefMacro{exp-java-num-vanilla-MIN-dup1}{32}
\DefMacro{exp-java-num-vanilla-MEDIAN-dup1}{709.00}
\DefMacro{exp-java-num-vanilla-STDEV-dup1}{1,773.96}
\DefMacro{exp-java-num-vanilla-CNT-dup1}{7}
\DefMacro{exp-java-num-unit-AVG-dup1}{1,454.14}
\DefMacro{exp-java-num-unit-SUM-dup1}{10,179}
\DefMacro{exp-java-num-unit-MAX-dup1}{5,022}
\DefMacro{exp-java-num-unit-MIN-dup1}{32}
\DefMacro{exp-java-num-unit-MEDIAN-dup1}{709.00}
\DefMacro{exp-java-num-unit-STDEV-dup1}{1,773.96}
\DefMacro{exp-java-num-unit-CNT-dup1}{7}
\DefMacro{exp-java-num-inline-AVG-dup1}{1.43}
\DefMacro{exp-java-num-inline-SUM-dup1}{10}
\DefMacro{exp-java-num-inline-MAX-dup1}{2}
\DefMacro{exp-java-num-inline-MIN-dup1}{1}
\DefMacro{exp-java-num-inline-MEDIAN-dup1}{1.00}
\DefMacro{exp-java-num-inline-STDEV-dup1}{0.49}
\DefMacro{exp-java-num-inline-CNT-dup1}{7}
\DefMacro{exp-java-num-unit-and-inline-AVG-dup1}{1,455.57}
\DefMacro{exp-java-num-unit-and-inline-SUM-dup1}{10,189}
\DefMacro{exp-java-num-unit-and-inline-MAX-dup1}{5,024}
\DefMacro{exp-java-num-unit-and-inline-MIN-dup1}{34}
\DefMacro{exp-java-num-unit-and-inline-MEDIAN-dup1}{710.00}
\DefMacro{exp-java-num-unit-and-inline-STDEV-dup1}{1,774.02}
\DefMacro{exp-java-num-unit-and-inline-CNT-dup1}{7}
\DefMacro{exp-java-timept-vanilla-AVG-dup1}{0.125}
\DefMacro{exp-java-timept-vanilla-SUM-dup1}{0.878}
\DefMacro{exp-java-timept-vanilla-MAX-dup1}{0.257}
\DefMacro{exp-java-timept-vanilla-MIN-dup1}{0.009}
\DefMacro{exp-java-timept-vanilla-MEDIAN-dup1}{0.114}
\DefMacro{exp-java-timept-vanilla-STDEV-dup1}{0.082}
\DefMacro{exp-java-timept-vanilla-CNT-dup1}{7}
\DefMacro{exp-java-timept-unit-AVG-dup1}{0.127}
\DefMacro{exp-java-timept-unit-SUM-dup1}{0.892}
\DefMacro{exp-java-timept-unit-MAX-dup1}{0.257}
\DefMacro{exp-java-timept-unit-MIN-dup1}{0.009}
\DefMacro{exp-java-timept-unit-MEDIAN-dup1}{0.115}
\DefMacro{exp-java-timept-unit-STDEV-dup1}{0.081}
\DefMacro{exp-java-timept-unit-CNT-dup1}{7}
\DefMacro{exp-java-timept-inline-AVG-dup1}{0.574}
\DefMacro{exp-java-timept-inline-SUM-dup1}{4.017}
\DefMacro{exp-java-timept-inline-MAX-dup1}{0.822}
\DefMacro{exp-java-timept-inline-MIN-dup1}{0.325}
\DefMacro{exp-java-timept-inline-MEDIAN-dup1}{0.670}
\DefMacro{exp-java-timept-inline-STDEV-dup1}{0.201}
\DefMacro{exp-java-timept-inline-CNT-dup1}{7}
\DefMacro{exp-java-timept-unit-and-inline-AVG-dup1}{0.131}
\DefMacro{exp-java-timept-unit-and-inline-SUM-dup1}{0.917}
\DefMacro{exp-java-timept-unit-and-inline-MAX-dup1}{0.258}
\DefMacro{exp-java-timept-unit-and-inline-MIN-dup1}{0.009}
\DefMacro{exp-java-timept-unit-and-inline-MEDIAN-dup1}{0.125}
\DefMacro{exp-java-timept-unit-and-inline-STDEV-dup1}{0.081}
\DefMacro{exp-java-timept-unit-and-inline-CNT-dup1}{7}
\DefMacro{exp-java-overhead-unit-AVG-dup1}{0.022}
\DefMacro{exp-java-overhead-unit-SUM-dup1}{0.155}
\DefMacro{exp-java-overhead-unit-MAX-dup1}{0.134}
\DefMacro{exp-java-overhead-unit-MIN-dup1}{-0.007}
\DefMacro{exp-java-overhead-unit-MEDIAN-dup1}{0.002}
\DefMacro{exp-java-overhead-unit-STDEV-dup1}{0.047}
\DefMacro{exp-java-overhead-unit-CNT-dup1}{7}
\DefMacro{exp-java-overhead-unit-and-inline-AVG-dup1}{0.076}
\DefMacro{exp-java-overhead-unit-and-inline-SUM-dup1}{0.535}
\DefMacro{exp-java-overhead-unit-and-inline-MAX-dup1}{0.145}
\DefMacro{exp-java-overhead-unit-and-inline-MIN-dup1}{0.002}
\DefMacro{exp-java-overhead-unit-and-inline-MEDIAN-dup1}{0.094}
\DefMacro{exp-java-overhead-unit-and-inline-STDEV-dup1}{0.062}
\DefMacro{exp-java-overhead-unit-and-inline-CNT-dup1}{7}
\DefMacro{exp-java-timept-vanilla-MACROAVG-dup1}{0.104}
\DefMacro{exp-java-timept-unit-MACROAVG-dup1}{0.105}
\DefMacro{exp-java-timept-inline-MACROAVG-dup1}{0.506}
\DefMacro{exp-java-timept-unit-and-inline-MACROAVG-dup1}{0.105}
\DefMacro{exp-java-overhead-unit-MACROAVG-dup1}{0.009}
\DefMacro{exp-java-overhead-unit-and-inline-MACROAVG-dup1}{0.014}
\DefMacro{exp-java-alibaba_fastjson-time-vanilla-dup10}{44.99}
\DefMacro{exp-java-alibaba_fastjson-time-unit-dup10}{44.73}
\DefMacro{exp-java-alibaba_fastjson-time-inline-dup10}{0.69}
\DefMacro{exp-java-alibaba_fastjson-time-unit-and-inline-dup10}{45.42}
\DefMacro{exp-java-alibaba_fastjson-num-vanilla-dup10}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-unit-dup10}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-inline-dup10}{20}
\DefMacro{exp-java-alibaba_fastjson-num-unit-and-inline-dup10}{5,042}
\DefMacro{exp-java-alibaba_fastjson-timept-vanilla-dup10}{0.009}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-dup10}{0.009}
\DefMacro{exp-java-alibaba_fastjson-timept-inline-dup10}{0.035}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-and-inline-dup10}{0.009}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-dup10}{-0.006}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-and-inline-dup10}{0.010}
\DefMacro{exp-java-alibaba_nacos-time-vanilla-dup10}{248.65}
\DefMacro{exp-java-alibaba_nacos-time-unit-dup10}{249.20}
\DefMacro{exp-java-alibaba_nacos-time-inline-dup10}{0.67}
\DefMacro{exp-java-alibaba_nacos-time-unit-and-inline-dup10}{249.87}
\DefMacro{exp-java-alibaba_nacos-num-vanilla-dup10}{971}
\DefMacro{exp-java-alibaba_nacos-num-unit-dup10}{971}
\DefMacro{exp-java-alibaba_nacos-num-inline-dup10}{10}
\DefMacro{exp-java-alibaba_nacos-num-unit-and-inline-dup10}{981}
\DefMacro{exp-java-alibaba_nacos-timept-vanilla-dup10}{0.256}
\DefMacro{exp-java-alibaba_nacos-timept-unit-dup10}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-inline-dup10}{0.067}
\DefMacro{exp-java-alibaba_nacos-timept-unit-and-inline-dup10}{0.255}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-dup10}{0.002}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-and-inline-dup10}{0.005}
\DefMacro{exp-java-apache_dubbo-time-vanilla-dup10}{678.61}
\DefMacro{exp-java-apache_dubbo-time-unit-dup10}{680.85}
\DefMacro{exp-java-apache_dubbo-time-inline-dup10}{0.74}
\DefMacro{exp-java-apache_dubbo-time-unit-and-inline-dup10}{681.59}
\DefMacro{exp-java-apache_dubbo-num-vanilla-dup10}{3,180}
\DefMacro{exp-java-apache_dubbo-num-unit-dup10}{3,180}
\DefMacro{exp-java-apache_dubbo-num-inline-dup10}{10}
\DefMacro{exp-java-apache_dubbo-num-unit-and-inline-dup10}{3,190}
\DefMacro{exp-java-apache_dubbo-timept-vanilla-dup10}{0.213}
\DefMacro{exp-java-apache_dubbo-timept-unit-dup10}{0.214}
\DefMacro{exp-java-apache_dubbo-timept-inline-dup10}{0.074}
\DefMacro{exp-java-apache_dubbo-timept-unit-and-inline-dup10}{0.214}
\DefMacro{exp-java-apache_dubbo-overhead-unit-dup10}{0.003}
\DefMacro{exp-java-apache_dubbo-overhead-unit-and-inline-dup10}{0.004}
\DefMacro{exp-java-apache_kafka-time-vanilla-dup10}{9.91}
\DefMacro{exp-java-apache_kafka-time-unit-dup10}{10.08}
\DefMacro{exp-java-apache_kafka-time-inline-dup10}{0.71}
\DefMacro{exp-java-apache_kafka-time-unit-and-inline-dup10}{10.79}
\DefMacro{exp-java-apache_kafka-num-vanilla-dup10}{221}
\DefMacro{exp-java-apache_kafka-num-unit-dup10}{221}
\DefMacro{exp-java-apache_kafka-num-inline-dup10}{10}
\DefMacro{exp-java-apache_kafka-num-unit-and-inline-dup10}{231}
\DefMacro{exp-java-apache_kafka-timept-vanilla-dup10}{0.045}
\DefMacro{exp-java-apache_kafka-timept-unit-dup10}{0.046}
\DefMacro{exp-java-apache_kafka-timept-inline-dup10}{0.071}
\DefMacro{exp-java-apache_kafka-timept-unit-and-inline-dup10}{0.047}
\DefMacro{exp-java-apache_kafka-overhead-unit-dup10}{0.018}
\DefMacro{exp-java-apache_kafka-overhead-unit-and-inline-dup10}{0.089}
\DefMacro{exp-java-apache_shardingsphere-time-vanilla-dup10}{5.09}
\DefMacro{exp-java-apache_shardingsphere-time-unit-dup10}{5.09}
\DefMacro{exp-java-apache_shardingsphere-time-inline-dup10}{0.68}
\DefMacro{exp-java-apache_shardingsphere-time-unit-and-inline-dup10}{5.76}
\DefMacro{exp-java-apache_shardingsphere-num-vanilla-dup10}{44}
\DefMacro{exp-java-apache_shardingsphere-num-unit-dup10}{44}
\DefMacro{exp-java-apache_shardingsphere-num-inline-dup10}{20}
\DefMacro{exp-java-apache_shardingsphere-num-unit-and-inline-dup10}{64}
\DefMacro{exp-java-apache_shardingsphere-timept-vanilla-dup10}{0.116}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-dup10}{0.116}
\DefMacro{exp-java-apache_shardingsphere-timept-inline-dup10}{0.034}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-and-inline-dup10}{0.090}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-dup10}{-0.000}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-and-inline-dup10}{0.133}
\DefMacro{exp-java-jenkinsci_jenkins-time-vanilla-dup10}{4.67}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-dup10}{4.70}
\DefMacro{exp-java-jenkinsci_jenkins-time-inline-dup10}{0.72}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-and-inline-dup10}{5.42}
\DefMacro{exp-java-jenkinsci_jenkins-num-vanilla-dup10}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-dup10}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-inline-dup10}{20}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-and-inline-dup10}{52}
\DefMacro{exp-java-jenkinsci_jenkins-timept-vanilla-dup10}{0.146}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-dup10}{0.147}
\DefMacro{exp-java-jenkinsci_jenkins-timept-inline-dup10}{0.036}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-and-inline-dup10}{0.104}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-dup10}{0.006}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-and-inline-dup10}{0.160}
\DefMacro{exp-java-skylot_jadx-time-vanilla-dup10}{67.43}
\DefMacro{exp-java-skylot_jadx-time-unit-dup10}{65.82}
\DefMacro{exp-java-skylot_jadx-time-inline-dup10}{0.71}
\DefMacro{exp-java-skylot_jadx-time-unit-and-inline-dup10}{66.52}
\DefMacro{exp-java-skylot_jadx-num-vanilla-dup10}{709}
\DefMacro{exp-java-skylot_jadx-num-unit-dup10}{709}
\DefMacro{exp-java-skylot_jadx-num-inline-dup10}{10}
\DefMacro{exp-java-skylot_jadx-num-unit-and-inline-dup10}{719}
\DefMacro{exp-java-skylot_jadx-timept-vanilla-dup10}{0.095}
\DefMacro{exp-java-skylot_jadx-timept-unit-dup10}{0.093}
\DefMacro{exp-java-skylot_jadx-timept-inline-dup10}{0.071}
\DefMacro{exp-java-skylot_jadx-timept-unit-and-inline-dup10}{0.093}
\DefMacro{exp-java-skylot_jadx-overhead-unit-dup10}{-0.024}
\DefMacro{exp-java-skylot_jadx-overhead-unit-and-inline-dup10}{-0.014}
\DefMacro{exp-java-time-vanilla-AVG-dup10}{151.34}
\DefMacro{exp-java-time-vanilla-SUM-dup10}{1,059.36}
\DefMacro{exp-java-time-vanilla-MAX-dup10}{678.61}
\DefMacro{exp-java-time-vanilla-MIN-dup10}{4.67}
\DefMacro{exp-java-time-vanilla-MEDIAN-dup10}{44.99}
\DefMacro{exp-java-time-vanilla-STDEV-dup10}{229.51}
\DefMacro{exp-java-time-vanilla-CNT-dup10}{7}
\DefMacro{exp-java-time-unit-AVG-dup10}{151.50}
\DefMacro{exp-java-time-unit-SUM-dup10}{1,060.47}
\DefMacro{exp-java-time-unit-MAX-dup10}{680.85}
\DefMacro{exp-java-time-unit-MIN-dup10}{4.70}
\DefMacro{exp-java-time-unit-MEDIAN-dup10}{44.73}
\DefMacro{exp-java-time-unit-STDEV-dup10}{230.37}
\DefMacro{exp-java-time-unit-CNT-dup10}{7}
\DefMacro{exp-java-time-inline-AVG-dup10}{0.70}
\DefMacro{exp-java-time-inline-SUM-dup10}{4.91}
\DefMacro{exp-java-time-inline-MAX-dup10}{0.74}
\DefMacro{exp-java-time-inline-MIN-dup10}{0.67}
\DefMacro{exp-java-time-inline-MEDIAN-dup10}{0.71}
\DefMacro{exp-java-time-inline-STDEV-dup10}{0.02}
\DefMacro{exp-java-time-inline-CNT-dup10}{7}
\DefMacro{exp-java-time-unit-and-inline-AVG-dup10}{152.20}
\DefMacro{exp-java-time-unit-and-inline-SUM-dup10}{1,065.38}
\DefMacro{exp-java-time-unit-and-inline-MAX-dup10}{681.59}
\DefMacro{exp-java-time-unit-and-inline-MIN-dup10}{5.42}
\DefMacro{exp-java-time-unit-and-inline-MEDIAN-dup10}{45.42}
\DefMacro{exp-java-time-unit-and-inline-STDEV-dup10}{230.38}
\DefMacro{exp-java-time-unit-and-inline-CNT-dup10}{7}
\DefMacro{exp-java-num-vanilla-AVG-dup10}{1,454.14}
\DefMacro{exp-java-num-vanilla-SUM-dup10}{10,179}
\DefMacro{exp-java-num-vanilla-MAX-dup10}{5,022}
\DefMacro{exp-java-num-vanilla-MIN-dup10}{32}
\DefMacro{exp-java-num-vanilla-MEDIAN-dup10}{709.00}
\DefMacro{exp-java-num-vanilla-STDEV-dup10}{1,773.96}
\DefMacro{exp-java-num-vanilla-CNT-dup10}{7}
\DefMacro{exp-java-num-unit-AVG-dup10}{1,454.14}
\DefMacro{exp-java-num-unit-SUM-dup10}{10,179}
\DefMacro{exp-java-num-unit-MAX-dup10}{5,022}
\DefMacro{exp-java-num-unit-MIN-dup10}{32}
\DefMacro{exp-java-num-unit-MEDIAN-dup10}{709.00}
\DefMacro{exp-java-num-unit-STDEV-dup10}{1,773.96}
\DefMacro{exp-java-num-unit-CNT-dup10}{7}
\DefMacro{exp-java-num-inline-AVG-dup10}{14.29}
\DefMacro{exp-java-num-inline-SUM-dup10}{100}
\DefMacro{exp-java-num-inline-MAX-dup10}{20}
\DefMacro{exp-java-num-inline-MIN-dup10}{10}
\DefMacro{exp-java-num-inline-MEDIAN-dup10}{10.00}
\DefMacro{exp-java-num-inline-STDEV-dup10}{4.95}
\DefMacro{exp-java-num-inline-CNT-dup10}{7}
\DefMacro{exp-java-num-unit-and-inline-AVG-dup10}{1,468.43}
\DefMacro{exp-java-num-unit-and-inline-SUM-dup10}{10,279}
\DefMacro{exp-java-num-unit-and-inline-MAX-dup10}{5,042}
\DefMacro{exp-java-num-unit-and-inline-MIN-dup10}{52}
\DefMacro{exp-java-num-unit-and-inline-MEDIAN-dup10}{719.00}
\DefMacro{exp-java-num-unit-and-inline-STDEV-dup10}{1,774.56}
\DefMacro{exp-java-num-unit-and-inline-CNT-dup10}{7}
\DefMacro{exp-java-timept-vanilla-AVG-dup10}{0.126}
\DefMacro{exp-java-timept-vanilla-SUM-dup10}{0.880}
\DefMacro{exp-java-timept-vanilla-MAX-dup10}{0.256}
\DefMacro{exp-java-timept-vanilla-MIN-dup10}{0.009}
\DefMacro{exp-java-timept-vanilla-MEDIAN-dup10}{0.116}
\DefMacro{exp-java-timept-vanilla-STDEV-dup10}{0.081}
\DefMacro{exp-java-timept-vanilla-CNT-dup10}{7}
\DefMacro{exp-java-timept-unit-AVG-dup10}{0.126}
\DefMacro{exp-java-timept-unit-SUM-dup10}{0.881}
\DefMacro{exp-java-timept-unit-MAX-dup10}{0.257}
\DefMacro{exp-java-timept-unit-MIN-dup10}{0.009}
\DefMacro{exp-java-timept-unit-MEDIAN-dup10}{0.116}
\DefMacro{exp-java-timept-unit-STDEV-dup10}{0.082}
\DefMacro{exp-java-timept-unit-CNT-dup10}{7}
\DefMacro{exp-java-timept-inline-AVG-dup10}{0.055}
\DefMacro{exp-java-timept-inline-SUM-dup10}{0.387}
\DefMacro{exp-java-timept-inline-MAX-dup10}{0.074}
\DefMacro{exp-java-timept-inline-MIN-dup10}{0.034}
\DefMacro{exp-java-timept-inline-MEDIAN-dup10}{0.067}
\DefMacro{exp-java-timept-inline-STDEV-dup10}{0.018}
\DefMacro{exp-java-timept-inline-CNT-dup10}{7}
\DefMacro{exp-java-timept-unit-and-inline-AVG-dup10}{0.116}
\DefMacro{exp-java-timept-unit-and-inline-SUM-dup10}{0.811}
\DefMacro{exp-java-timept-unit-and-inline-MAX-dup10}{0.255}
\DefMacro{exp-java-timept-unit-and-inline-MIN-dup10}{0.009}
\DefMacro{exp-java-timept-unit-and-inline-MEDIAN-dup10}{0.093}
\DefMacro{exp-java-timept-unit-and-inline-STDEV-dup10}{0.081}
\DefMacro{exp-java-timept-unit-and-inline-CNT-dup10}{7}
\DefMacro{exp-java-overhead-unit-AVG-dup10}{-0.000}
\DefMacro{exp-java-overhead-unit-SUM-dup10}{-0.000}
\DefMacro{exp-java-overhead-unit-MAX-dup10}{0.018}
\DefMacro{exp-java-overhead-unit-MIN-dup10}{-0.024}
\DefMacro{exp-java-overhead-unit-MEDIAN-dup10}{0.002}
\DefMacro{exp-java-overhead-unit-STDEV-dup10}{0.012}
\DefMacro{exp-java-overhead-unit-CNT-dup10}{7}
\DefMacro{exp-java-overhead-unit-and-inline-AVG-dup10}{0.055}
\DefMacro{exp-java-overhead-unit-and-inline-SUM-dup10}{0.388}
\DefMacro{exp-java-overhead-unit-and-inline-MAX-dup10}{0.160}
\DefMacro{exp-java-overhead-unit-and-inline-MIN-dup10}{-0.014}
\DefMacro{exp-java-overhead-unit-and-inline-MEDIAN-dup10}{0.010}
\DefMacro{exp-java-overhead-unit-and-inline-STDEV-dup10}{0.066}
\DefMacro{exp-java-overhead-unit-and-inline-CNT-dup10}{7}
\DefMacro{exp-java-timept-vanilla-MACROAVG-dup10}{0.104}
\DefMacro{exp-java-timept-unit-MACROAVG-dup10}{0.104}
\DefMacro{exp-java-timept-inline-MACROAVG-dup10}{0.049}
\DefMacro{exp-java-timept-unit-and-inline-MACROAVG-dup10}{0.104}
\DefMacro{exp-java-overhead-unit-MACROAVG-dup10}{0.001}
\DefMacro{exp-java-overhead-unit-and-inline-MACROAVG-dup10}{0.006}
\DefMacro{exp-java-alibaba_fastjson-time-vanilla-dup100}{44.86}
\DefMacro{exp-java-alibaba_fastjson-time-unit-dup100}{52.40}
\DefMacro{exp-java-alibaba_fastjson-time-inline-dup100}{0.72}
\DefMacro{exp-java-alibaba_fastjson-time-unit-and-inline-dup100}{53.13}
\DefMacro{exp-java-alibaba_fastjson-num-vanilla-dup100}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-unit-dup100}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-inline-dup100}{200}
\DefMacro{exp-java-alibaba_fastjson-num-unit-and-inline-dup100}{5,222}
\DefMacro{exp-java-alibaba_fastjson-timept-vanilla-dup100}{0.009}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-dup100}{0.010}
\DefMacro{exp-java-alibaba_fastjson-timept-inline-dup100}{0.004}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-and-inline-dup100}{0.010}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-dup100}{0.168}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-and-inline-dup100}{0.184}
\DefMacro{exp-java-alibaba_nacos-time-vanilla-dup100}{249.59}
\DefMacro{exp-java-alibaba_nacos-time-unit-dup100}{249.86}
\DefMacro{exp-java-alibaba_nacos-time-inline-dup100}{0.69}
\DefMacro{exp-java-alibaba_nacos-time-unit-and-inline-dup100}{250.54}
\DefMacro{exp-java-alibaba_nacos-num-vanilla-dup100}{971}
\DefMacro{exp-java-alibaba_nacos-num-unit-dup100}{971}
\DefMacro{exp-java-alibaba_nacos-num-inline-dup100}{100}
\DefMacro{exp-java-alibaba_nacos-num-unit-and-inline-dup100}{1,071}
\DefMacro{exp-java-alibaba_nacos-timept-vanilla-dup100}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-unit-dup100}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-inline-dup100}{0.007}
\DefMacro{exp-java-alibaba_nacos-timept-unit-and-inline-dup100}{0.234}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-dup100}{0.001}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-and-inline-dup100}{0.004}
\DefMacro{exp-java-apache_dubbo-time-vanilla-dup100}{678.24}
\DefMacro{exp-java-apache_dubbo-time-unit-dup100}{680.08}
\DefMacro{exp-java-apache_dubbo-time-inline-dup100}{0.74}
\DefMacro{exp-java-apache_dubbo-time-unit-and-inline-dup100}{680.81}
\DefMacro{exp-java-apache_dubbo-num-vanilla-dup100}{3,180}
\DefMacro{exp-java-apache_dubbo-num-unit-dup100}{3,180}
\DefMacro{exp-java-apache_dubbo-num-inline-dup100}{100}
\DefMacro{exp-java-apache_dubbo-num-unit-and-inline-dup100}{3,280}
\DefMacro{exp-java-apache_dubbo-timept-vanilla-dup100}{0.213}
\DefMacro{exp-java-apache_dubbo-timept-unit-dup100}{0.214}
\DefMacro{exp-java-apache_dubbo-timept-inline-dup100}{0.007}
\DefMacro{exp-java-apache_dubbo-timept-unit-and-inline-dup100}{0.208}
\DefMacro{exp-java-apache_dubbo-overhead-unit-dup100}{0.003}
\DefMacro{exp-java-apache_dubbo-overhead-unit-and-inline-dup100}{0.004}
\DefMacro{exp-java-apache_kafka-time-vanilla-dup100}{9.93}
\DefMacro{exp-java-apache_kafka-time-unit-dup100}{10.13}
\DefMacro{exp-java-apache_kafka-time-inline-dup100}{0.72}
\DefMacro{exp-java-apache_kafka-time-unit-and-inline-dup100}{10.86}
\DefMacro{exp-java-apache_kafka-num-vanilla-dup100}{221}
\DefMacro{exp-java-apache_kafka-num-unit-dup100}{221}
\DefMacro{exp-java-apache_kafka-num-inline-dup100}{100}
\DefMacro{exp-java-apache_kafka-num-unit-and-inline-dup100}{321}
\DefMacro{exp-java-apache_kafka-timept-vanilla-dup100}{0.045}
\DefMacro{exp-java-apache_kafka-timept-unit-dup100}{0.046}
\DefMacro{exp-java-apache_kafka-timept-inline-dup100}{0.007}
\DefMacro{exp-java-apache_kafka-timept-unit-and-inline-dup100}{0.034}
\DefMacro{exp-java-apache_kafka-overhead-unit-dup100}{0.021}
\DefMacro{exp-java-apache_kafka-overhead-unit-and-inline-dup100}{0.094}
\DefMacro{exp-java-apache_shardingsphere-time-vanilla-dup100}{5.08}
\DefMacro{exp-java-apache_shardingsphere-time-unit-dup100}{5.12}
\DefMacro{exp-java-apache_shardingsphere-time-inline-dup100}{0.72}
\DefMacro{exp-java-apache_shardingsphere-time-unit-and-inline-dup100}{5.84}
\DefMacro{exp-java-apache_shardingsphere-num-vanilla-dup100}{44}
\DefMacro{exp-java-apache_shardingsphere-num-unit-dup100}{44}
\DefMacro{exp-java-apache_shardingsphere-num-inline-dup100}{200}
\DefMacro{exp-java-apache_shardingsphere-num-unit-and-inline-dup100}{244}
\DefMacro{exp-java-apache_shardingsphere-timept-vanilla-dup100}{0.116}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-dup100}{0.116}
\DefMacro{exp-java-apache_shardingsphere-timept-inline-dup100}{0.004}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-and-inline-dup100}{0.024}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-dup100}{0.007}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-and-inline-dup100}{0.149}
\DefMacro{exp-java-jenkinsci_jenkins-time-vanilla-dup100}{4.65}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-dup100}{4.68}
\DefMacro{exp-java-jenkinsci_jenkins-time-inline-dup100}{0.72}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-and-inline-dup100}{5.40}
\DefMacro{exp-java-jenkinsci_jenkins-num-vanilla-dup100}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-dup100}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-inline-dup100}{200}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-and-inline-dup100}{232}
\DefMacro{exp-java-jenkinsci_jenkins-timept-vanilla-dup100}{0.145}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-dup100}{0.146}
\DefMacro{exp-java-jenkinsci_jenkins-timept-inline-dup100}{0.004}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-and-inline-dup100}{0.023}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-dup100}{0.006}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-and-inline-dup100}{0.162}
\DefMacro{exp-java-skylot_jadx-time-vanilla-dup100}{66.76}
\DefMacro{exp-java-skylot_jadx-time-unit-dup100}{66.17}
\DefMacro{exp-java-skylot_jadx-time-inline-dup100}{0.74}
\DefMacro{exp-java-skylot_jadx-time-unit-and-inline-dup100}{66.91}
\DefMacro{exp-java-skylot_jadx-num-vanilla-dup100}{709}
\DefMacro{exp-java-skylot_jadx-num-unit-dup100}{709}
\DefMacro{exp-java-skylot_jadx-num-inline-dup100}{100}
\DefMacro{exp-java-skylot_jadx-num-unit-and-inline-dup100}{809}
\DefMacro{exp-java-skylot_jadx-timept-vanilla-dup100}{0.094}
\DefMacro{exp-java-skylot_jadx-timept-unit-dup100}{0.093}
\DefMacro{exp-java-skylot_jadx-timept-inline-dup100}{0.007}
\DefMacro{exp-java-skylot_jadx-timept-unit-and-inline-dup100}{0.083}
\DefMacro{exp-java-skylot_jadx-overhead-unit-dup100}{-0.009}
\DefMacro{exp-java-skylot_jadx-overhead-unit-and-inline-dup100}{0.002}
\DefMacro{exp-java-time-vanilla-AVG-dup100}{151.30}
\DefMacro{exp-java-time-vanilla-SUM-dup100}{1,059.11}
\DefMacro{exp-java-time-vanilla-MAX-dup100}{678.24}
\DefMacro{exp-java-time-vanilla-MIN-dup100}{4.65}
\DefMacro{exp-java-time-vanilla-MEDIAN-dup100}{44.86}
\DefMacro{exp-java-time-vanilla-STDEV-dup100}{229.49}
\DefMacro{exp-java-time-vanilla-CNT-dup100}{7}
\DefMacro{exp-java-time-unit-AVG-dup100}{152.63}
\DefMacro{exp-java-time-unit-SUM-dup100}{1,068.44}
\DefMacro{exp-java-time-unit-MAX-dup100}{680.08}
\DefMacro{exp-java-time-unit-MIN-dup100}{4.68}
\DefMacro{exp-java-time-unit-MEDIAN-dup100}{52.40}
\DefMacro{exp-java-time-unit-STDEV-dup100}{229.64}
\DefMacro{exp-java-time-unit-CNT-dup100}{7}
\DefMacro{exp-java-time-inline-AVG-dup100}{0.72}
\DefMacro{exp-java-time-inline-SUM-dup100}{5.06}
\DefMacro{exp-java-time-inline-MAX-dup100}{0.74}
\DefMacro{exp-java-time-inline-MIN-dup100}{0.69}
\DefMacro{exp-java-time-inline-MEDIAN-dup100}{0.72}
\DefMacro{exp-java-time-inline-STDEV-dup100}{0.01}
\DefMacro{exp-java-time-inline-CNT-dup100}{7}
\DefMacro{exp-java-time-unit-and-inline-AVG-dup100}{153.36}
\DefMacro{exp-java-time-unit-and-inline-SUM-dup100}{1,073.50}
\DefMacro{exp-java-time-unit-and-inline-MAX-dup100}{680.81}
\DefMacro{exp-java-time-unit-and-inline-MIN-dup100}{5.40}
\DefMacro{exp-java-time-unit-and-inline-MEDIAN-dup100}{53.13}
\DefMacro{exp-java-time-unit-and-inline-STDEV-dup100}{229.64}
\DefMacro{exp-java-time-unit-and-inline-CNT-dup100}{7}
\DefMacro{exp-java-num-vanilla-AVG-dup100}{1,454.14}
\DefMacro{exp-java-num-vanilla-SUM-dup100}{10,179}
\DefMacro{exp-java-num-vanilla-MAX-dup100}{5,022}
\DefMacro{exp-java-num-vanilla-MIN-dup100}{32}
\DefMacro{exp-java-num-vanilla-MEDIAN-dup100}{709.00}
\DefMacro{exp-java-num-vanilla-STDEV-dup100}{1,773.96}
\DefMacro{exp-java-num-vanilla-CNT-dup100}{7}
\DefMacro{exp-java-num-unit-AVG-dup100}{1,454.14}
\DefMacro{exp-java-num-unit-SUM-dup100}{10,179}
\DefMacro{exp-java-num-unit-MAX-dup100}{5,022}
\DefMacro{exp-java-num-unit-MIN-dup100}{32}
\DefMacro{exp-java-num-unit-MEDIAN-dup100}{709.00}
\DefMacro{exp-java-num-unit-STDEV-dup100}{1,773.96}
\DefMacro{exp-java-num-unit-CNT-dup100}{7}
\DefMacro{exp-java-num-inline-AVG-dup100}{142.86}
\DefMacro{exp-java-num-inline-SUM-dup100}{1,000}
\DefMacro{exp-java-num-inline-MAX-dup100}{200}
\DefMacro{exp-java-num-inline-MIN-dup100}{100}
\DefMacro{exp-java-num-inline-MEDIAN-dup100}{100.00}
\DefMacro{exp-java-num-inline-STDEV-dup100}{49.49}
\DefMacro{exp-java-num-inline-CNT-dup100}{7}
\DefMacro{exp-java-num-unit-and-inline-AVG-dup100}{1,597.00}
\DefMacro{exp-java-num-unit-and-inline-SUM-dup100}{11,179}
\DefMacro{exp-java-num-unit-and-inline-MAX-dup100}{5,222}
\DefMacro{exp-java-num-unit-and-inline-MIN-dup100}{232}
\DefMacro{exp-java-num-unit-and-inline-MEDIAN-dup100}{809.00}
\DefMacro{exp-java-num-unit-and-inline-STDEV-dup100}{1,780.56}
\DefMacro{exp-java-num-unit-and-inline-CNT-dup100}{7}
\DefMacro{exp-java-timept-vanilla-AVG-dup100}{0.126}
\DefMacro{exp-java-timept-vanilla-SUM-dup100}{0.879}
\DefMacro{exp-java-timept-vanilla-MAX-dup100}{0.257}
\DefMacro{exp-java-timept-vanilla-MIN-dup100}{0.009}
\DefMacro{exp-java-timept-vanilla-MEDIAN-dup100}{0.116}
\DefMacro{exp-java-timept-vanilla-STDEV-dup100}{0.082}
\DefMacro{exp-java-timept-vanilla-CNT-dup100}{7}
\DefMacro{exp-java-timept-unit-AVG-dup100}{0.126}
\DefMacro{exp-java-timept-unit-SUM-dup100}{0.883}
\DefMacro{exp-java-timept-unit-MAX-dup100}{0.257}
\DefMacro{exp-java-timept-unit-MIN-dup100}{0.010}
\DefMacro{exp-java-timept-unit-MEDIAN-dup100}{0.116}
\DefMacro{exp-java-timept-unit-STDEV-dup100}{0.081}
\DefMacro{exp-java-timept-unit-CNT-dup100}{7}
\DefMacro{exp-java-timept-inline-AVG-dup100}{0.006}
\DefMacro{exp-java-timept-inline-SUM-dup100}{0.040}
\DefMacro{exp-java-timept-inline-MAX-dup100}{0.007}
\DefMacro{exp-java-timept-inline-MIN-dup100}{0.004}
\DefMacro{exp-java-timept-inline-MEDIAN-dup100}{0.007}
\DefMacro{exp-java-timept-inline-STDEV-dup100}{0.002}
\DefMacro{exp-java-timept-inline-CNT-dup100}{7}
\DefMacro{exp-java-timept-unit-and-inline-AVG-dup100}{0.088}
\DefMacro{exp-java-timept-unit-and-inline-SUM-dup100}{0.615}
\DefMacro{exp-java-timept-unit-and-inline-MAX-dup100}{0.234}
\DefMacro{exp-java-timept-unit-and-inline-MIN-dup100}{0.010}
\DefMacro{exp-java-timept-unit-and-inline-MEDIAN-dup100}{0.034}
\DefMacro{exp-java-timept-unit-and-inline-STDEV-dup100}{0.087}
\DefMacro{exp-java-timept-unit-and-inline-CNT-dup100}{7}
\DefMacro{exp-java-overhead-unit-AVG-dup100}{0.028}
\DefMacro{exp-java-overhead-unit-SUM-dup100}{0.197}
\DefMacro{exp-java-overhead-unit-MAX-dup100}{0.168}
\DefMacro{exp-java-overhead-unit-MIN-dup100}{-0.009}
\DefMacro{exp-java-overhead-unit-MEDIAN-dup100}{0.006}
\DefMacro{exp-java-overhead-unit-STDEV-dup100}{0.058}
\DefMacro{exp-java-overhead-unit-CNT-dup100}{7}
\DefMacro{exp-java-overhead-unit-and-inline-AVG-dup100}{0.086}
\DefMacro{exp-java-overhead-unit-and-inline-SUM-dup100}{0.599}
\DefMacro{exp-java-overhead-unit-and-inline-MAX-dup100}{0.184}
\DefMacro{exp-java-overhead-unit-and-inline-MIN-dup100}{0.002}
\DefMacro{exp-java-overhead-unit-and-inline-MEDIAN-dup100}{0.094}
\DefMacro{exp-java-overhead-unit-and-inline-STDEV-dup100}{0.076}
\DefMacro{exp-java-overhead-unit-and-inline-CNT-dup100}{7}
\DefMacro{exp-java-timept-vanilla-MACROAVG-dup100}{0.104}
\DefMacro{exp-java-timept-unit-MACROAVG-dup100}{0.105}
\DefMacro{exp-java-timept-inline-MACROAVG-dup100}{0.005}
\DefMacro{exp-java-timept-unit-and-inline-MACROAVG-dup100}{0.096}
\DefMacro{exp-java-overhead-unit-MACROAVG-dup100}{0.009}
\DefMacro{exp-java-overhead-unit-and-inline-MACROAVG-dup100}{0.014}
\DefMacro{exp-java-alibaba_fastjson-time-vanilla-dup1000}{44.82}
\DefMacro{exp-java-alibaba_fastjson-time-unit-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-time-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-num-vanilla-dup1000}{5,022}
\DefMacro{exp-java-alibaba_fastjson-num-unit-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-num-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-timept-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_fastjson-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-alibaba_nacos-time-vanilla-dup1000}{249.34}
\DefMacro{exp-java-alibaba_nacos-time-unit-dup1000}{249.96}
\DefMacro{exp-java-alibaba_nacos-time-inline-dup1000}{0.71}
\DefMacro{exp-java-alibaba_nacos-time-unit-and-inline-dup1000}{250.67}
\DefMacro{exp-java-alibaba_nacos-num-vanilla-dup1000}{971}
\DefMacro{exp-java-alibaba_nacos-num-unit-dup1000}{971}
\DefMacro{exp-java-alibaba_nacos-num-inline-dup1000}{1,000}
\DefMacro{exp-java-alibaba_nacos-num-unit-and-inline-dup1000}{1,971}
\DefMacro{exp-java-alibaba_nacos-timept-vanilla-dup1000}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-unit-dup1000}{0.257}
\DefMacro{exp-java-alibaba_nacos-timept-inline-dup1000}{0.001}
\DefMacro{exp-java-alibaba_nacos-timept-unit-and-inline-dup1000}{0.127}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-dup1000}{0.003}
\DefMacro{exp-java-alibaba_nacos-overhead-unit-and-inline-dup1000}{0.005}
\DefMacro{exp-java-apache_dubbo-time-vanilla-dup1000}{678.03}
\DefMacro{exp-java-apache_dubbo-time-unit-dup1000}{679.09}
\DefMacro{exp-java-apache_dubbo-time-inline-dup1000}{0.71}
\DefMacro{exp-java-apache_dubbo-time-unit-and-inline-dup1000}{679.79}
\DefMacro{exp-java-apache_dubbo-num-vanilla-dup1000}{3,180}
\DefMacro{exp-java-apache_dubbo-num-unit-dup1000}{3,180}
\DefMacro{exp-java-apache_dubbo-num-inline-dup1000}{1,000}
\DefMacro{exp-java-apache_dubbo-num-unit-and-inline-dup1000}{4,180}
\DefMacro{exp-java-apache_dubbo-timept-vanilla-dup1000}{0.213}
\DefMacro{exp-java-apache_dubbo-timept-unit-dup1000}{0.214}
\DefMacro{exp-java-apache_dubbo-timept-inline-dup1000}{0.001}
\DefMacro{exp-java-apache_dubbo-timept-unit-and-inline-dup1000}{0.163}
\DefMacro{exp-java-apache_dubbo-overhead-unit-dup1000}{0.002}
\DefMacro{exp-java-apache_dubbo-overhead-unit-and-inline-dup1000}{0.003}
\DefMacro{exp-java-apache_kafka-time-vanilla-dup1000}{9.92}
\DefMacro{exp-java-apache_kafka-time-unit-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-time-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-num-vanilla-dup1000}{221}
\DefMacro{exp-java-apache_kafka-num-unit-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-num-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-timept-unit-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-timept-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-java-apache_kafka-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-java-apache_shardingsphere-time-vanilla-dup1000}{5.06}
\DefMacro{exp-java-apache_shardingsphere-time-unit-dup1000}{5.09}
\DefMacro{exp-java-apache_shardingsphere-time-inline-dup1000}{0.78}
\DefMacro{exp-java-apache_shardingsphere-time-unit-and-inline-dup1000}{5.87}
\DefMacro{exp-java-apache_shardingsphere-num-vanilla-dup1000}{44}
\DefMacro{exp-java-apache_shardingsphere-num-unit-dup1000}{44}
\DefMacro{exp-java-apache_shardingsphere-num-inline-dup1000}{2,000}
\DefMacro{exp-java-apache_shardingsphere-num-unit-and-inline-dup1000}{2,044}
\DefMacro{exp-java-apache_shardingsphere-timept-vanilla-dup1000}{0.115}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-dup1000}{0.116}
\DefMacro{exp-java-apache_shardingsphere-timept-inline-dup1000}{0.000}
\DefMacro{exp-java-apache_shardingsphere-timept-unit-and-inline-dup1000}{0.003}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-dup1000}{0.005}
\DefMacro{exp-java-apache_shardingsphere-overhead-unit-and-inline-dup1000}{0.160}
\DefMacro{exp-java-jenkinsci_jenkins-time-vanilla-dup1000}{4.70}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-dup1000}{4.67}
\DefMacro{exp-java-jenkinsci_jenkins-time-inline-dup1000}{0.71}
\DefMacro{exp-java-jenkinsci_jenkins-time-unit-and-inline-dup1000}{5.38}
\DefMacro{exp-java-jenkinsci_jenkins-num-vanilla-dup1000}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-dup1000}{32}
\DefMacro{exp-java-jenkinsci_jenkins-num-inline-dup1000}{2,000}
\DefMacro{exp-java-jenkinsci_jenkins-num-unit-and-inline-dup1000}{2,032}
\DefMacro{exp-java-jenkinsci_jenkins-timept-vanilla-dup1000}{0.147}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-dup1000}{0.146}
\DefMacro{exp-java-jenkinsci_jenkins-timept-inline-dup1000}{0.000}
\DefMacro{exp-java-jenkinsci_jenkins-timept-unit-and-inline-dup1000}{0.003}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-dup1000}{-0.006}
\DefMacro{exp-java-jenkinsci_jenkins-overhead-unit-and-inline-dup1000}{0.145}
\DefMacro{exp-java-skylot_jadx-time-vanilla-dup1000}{67.11}
\DefMacro{exp-java-skylot_jadx-time-unit-dup1000}{69.73}
\DefMacro{exp-java-skylot_jadx-time-inline-dup1000}{0.70}
\DefMacro{exp-java-skylot_jadx-time-unit-and-inline-dup1000}{70.44}
\DefMacro{exp-java-skylot_jadx-num-vanilla-dup1000}{709}
\DefMacro{exp-java-skylot_jadx-num-unit-dup1000}{709}
\DefMacro{exp-java-skylot_jadx-num-inline-dup1000}{1,000}
\DefMacro{exp-java-skylot_jadx-num-unit-and-inline-dup1000}{1,709}
\DefMacro{exp-java-skylot_jadx-timept-vanilla-dup1000}{0.095}
\DefMacro{exp-java-skylot_jadx-timept-unit-dup1000}{0.098}
\DefMacro{exp-java-skylot_jadx-timept-inline-dup1000}{0.001}
\DefMacro{exp-java-skylot_jadx-timept-unit-and-inline-dup1000}{0.041}
\DefMacro{exp-java-skylot_jadx-overhead-unit-dup1000}{0.039}
\DefMacro{exp-java-skylot_jadx-overhead-unit-and-inline-dup1000}{0.050}
\DefMacro{exp-java-time-vanilla-AVG-dup1000}{200.85}
\DefMacro{exp-java-time-vanilla-SUM-dup1000}{1,004.24}
\DefMacro{exp-java-time-vanilla-MAX-dup1000}{678.03}
\DefMacro{exp-java-time-vanilla-MIN-dup1000}{4.70}
\DefMacro{exp-java-time-vanilla-MEDIAN-dup1000}{67.11}
\DefMacro{exp-java-time-vanilla-STDEV-dup1000}{254.85}
\DefMacro{exp-java-time-vanilla-CNT-dup1000}{5}
\DefMacro{exp-java-time-unit-AVG-dup1000}{201.71}
\DefMacro{exp-java-time-unit-SUM-dup1000}{1,008.55}
\DefMacro{exp-java-time-unit-MAX-dup1000}{679.09}
\DefMacro{exp-java-time-unit-MIN-dup1000}{4.67}
\DefMacro{exp-java-time-unit-MEDIAN-dup1000}{69.73}
\DefMacro{exp-java-time-unit-STDEV-dup1000}{255.00}
\DefMacro{exp-java-time-unit-CNT-dup1000}{5}
\DefMacro{exp-java-time-inline-AVG-dup1000}{0.72}
\DefMacro{exp-java-time-inline-SUM-dup1000}{3.61}
\DefMacro{exp-java-time-inline-MAX-dup1000}{0.78}
\DefMacro{exp-java-time-inline-MIN-dup1000}{0.70}
\DefMacro{exp-java-time-inline-MEDIAN-dup1000}{0.71}
\DefMacro{exp-java-time-inline-STDEV-dup1000}{0.03}
\DefMacro{exp-java-time-inline-CNT-dup1000}{5}
\DefMacro{exp-java-time-unit-and-inline-AVG-dup1000}{202.43}
\DefMacro{exp-java-time-unit-and-inline-SUM-dup1000}{1,012.16}
\DefMacro{exp-java-time-unit-and-inline-MAX-dup1000}{679.79}
\DefMacro{exp-java-time-unit-and-inline-MIN-dup1000}{5.38}
\DefMacro{exp-java-time-unit-and-inline-MEDIAN-dup1000}{70.44}
\DefMacro{exp-java-time-unit-and-inline-STDEV-dup1000}{254.99}
\DefMacro{exp-java-time-unit-and-inline-CNT-dup1000}{5}
\DefMacro{exp-java-num-vanilla-AVG-dup1000}{987.20}
\DefMacro{exp-java-num-vanilla-SUM-dup1000}{4,936}
\DefMacro{exp-java-num-vanilla-MAX-dup1000}{3,180}
\DefMacro{exp-java-num-vanilla-MIN-dup1000}{32}
\DefMacro{exp-java-num-vanilla-MEDIAN-dup1000}{709.00}
\DefMacro{exp-java-num-vanilla-STDEV-dup1000}{1,156.55}
\DefMacro{exp-java-num-vanilla-CNT-dup1000}{5}
\DefMacro{exp-java-num-unit-AVG-dup1000}{987.20}
\DefMacro{exp-java-num-unit-SUM-dup1000}{4,936}
\DefMacro{exp-java-num-unit-MAX-dup1000}{3,180}
\DefMacro{exp-java-num-unit-MIN-dup1000}{32}
\DefMacro{exp-java-num-unit-MEDIAN-dup1000}{709.00}
\DefMacro{exp-java-num-unit-STDEV-dup1000}{1,156.55}
\DefMacro{exp-java-num-unit-CNT-dup1000}{5}
\DefMacro{exp-java-num-inline-AVG-dup1000}{1,400.00}
\DefMacro{exp-java-num-inline-SUM-dup1000}{7,000}
\DefMacro{exp-java-num-inline-MAX-dup1000}{2,000}
\DefMacro{exp-java-num-inline-MIN-dup1000}{1,000}
\DefMacro{exp-java-num-inline-MEDIAN-dup1000}{1,000.00}
\DefMacro{exp-java-num-inline-STDEV-dup1000}{489.90}
\DefMacro{exp-java-num-inline-CNT-dup1000}{5}
\DefMacro{exp-java-num-unit-and-inline-AVG-dup1000}{2,387.20}
\DefMacro{exp-java-num-unit-and-inline-SUM-dup1000}{11,936}
\DefMacro{exp-java-num-unit-and-inline-MAX-dup1000}{4,180}
\DefMacro{exp-java-num-unit-and-inline-MIN-dup1000}{1,709}
\DefMacro{exp-java-num-unit-and-inline-MEDIAN-dup1000}{2,032.00}
\DefMacro{exp-java-num-unit-and-inline-STDEV-dup1000}{904.57}
\DefMacro{exp-java-num-unit-and-inline-CNT-dup1000}{5}
\DefMacro{exp-java-timept-vanilla-AVG-dup1000}{0.165}
\DefMacro{exp-java-timept-vanilla-SUM-dup1000}{0.827}
\DefMacro{exp-java-timept-vanilla-MAX-dup1000}{0.257}
\DefMacro{exp-java-timept-vanilla-MIN-dup1000}{0.095}
\DefMacro{exp-java-timept-vanilla-MEDIAN-dup1000}{0.147}
\DefMacro{exp-java-timept-vanilla-STDEV-dup1000}{0.061}
\DefMacro{exp-java-timept-vanilla-CNT-dup1000}{5}
\DefMacro{exp-java-timept-unit-AVG-dup1000}{0.166}
\DefMacro{exp-java-timept-unit-SUM-dup1000}{0.831}
\DefMacro{exp-java-timept-unit-MAX-dup1000}{0.257}
\DefMacro{exp-java-timept-unit-MIN-dup1000}{0.098}
\DefMacro{exp-java-timept-unit-MEDIAN-dup1000}{0.146}
\DefMacro{exp-java-timept-unit-STDEV-dup1000}{0.060}
\DefMacro{exp-java-timept-unit-CNT-dup1000}{5}
\DefMacro{exp-java-timept-inline-AVG-dup1000}{0.001}
\DefMacro{exp-java-timept-inline-SUM-dup1000}{0.003}
\DefMacro{exp-java-timept-inline-MAX-dup1000}{0.001}
\DefMacro{exp-java-timept-inline-MIN-dup1000}{0.000}
\DefMacro{exp-java-timept-inline-MEDIAN-dup1000}{0.001}
\DefMacro{exp-java-timept-inline-STDEV-dup1000}{0.000}
\DefMacro{exp-java-timept-inline-CNT-dup1000}{5}
\DefMacro{exp-java-timept-unit-and-inline-AVG-dup1000}{0.067}
\DefMacro{exp-java-timept-unit-and-inline-SUM-dup1000}{0.337}
\DefMacro{exp-java-timept-unit-and-inline-MAX-dup1000}{0.163}
\DefMacro{exp-java-timept-unit-and-inline-MIN-dup1000}{0.003}
\DefMacro{exp-java-timept-unit-and-inline-MEDIAN-dup1000}{0.041}
\DefMacro{exp-java-timept-unit-and-inline-STDEV-dup1000}{0.066}
\DefMacro{exp-java-timept-unit-and-inline-CNT-dup1000}{5}
\DefMacro{exp-java-overhead-unit-AVG-dup1000}{0.009}
\DefMacro{exp-java-overhead-unit-SUM-dup1000}{0.043}
\DefMacro{exp-java-overhead-unit-MAX-dup1000}{0.039}
\DefMacro{exp-java-overhead-unit-MIN-dup1000}{-0.006}
\DefMacro{exp-java-overhead-unit-MEDIAN-dup1000}{0.003}
\DefMacro{exp-java-overhead-unit-STDEV-dup1000}{0.016}
\DefMacro{exp-java-overhead-unit-CNT-dup1000}{5}
\DefMacro{exp-java-overhead-unit-and-inline-AVG-dup1000}{0.073}
\DefMacro{exp-java-overhead-unit-and-inline-SUM-dup1000}{0.363}
\DefMacro{exp-java-overhead-unit-and-inline-MAX-dup1000}{0.160}
\DefMacro{exp-java-overhead-unit-and-inline-MIN-dup1000}{0.003}
\DefMacro{exp-java-overhead-unit-and-inline-MEDIAN-dup1000}{0.050}
\DefMacro{exp-java-overhead-unit-and-inline-STDEV-dup1000}{0.068}
\DefMacro{exp-java-overhead-unit-and-inline-CNT-dup1000}{5}
\DefMacro{exp-java-timept-vanilla-MACROAVG-dup1000}{0.203}
\DefMacro{exp-java-timept-unit-MACROAVG-dup1000}{0.204}
\DefMacro{exp-java-timept-inline-MACROAVG-dup1000}{0.001}
\DefMacro{exp-java-timept-unit-and-inline-MACROAVG-dup1000}{0.085}
\DefMacro{exp-java-overhead-unit-MACROAVG-dup1000}{0.004}
\DefMacro{exp-java-overhead-unit-and-inline-MACROAVG-dup1000}{0.008}


==> tables/data-exp-integrated-python.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-python-RaRe-Technologies_gensim-time-vanilla-dup1}{224.85}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-dup1}{226.74}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-inline-dup1}{0.53}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-and-inline-dup1}{227.27}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-vanilla-dup1}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-dup1}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-inline-dup1}{2}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-and-inline-dup1}{969}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-vanilla-dup1}{0.233}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-dup1}{0.234}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-inline-dup1}{0.266}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-and-inline-dup1}{0.235}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-dup1}{0.008}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-and-inline-dup1}{0.011}
\DefMacro{exp-python-Textualize_rich-time-vanilla-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-vanilla-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-vanilla-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-dup1}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-bokeh_bokeh-time-vanilla-dup1}{60.76}
\DefMacro{exp-python-bokeh_bokeh-time-unit-dup1}{60.67}
\DefMacro{exp-python-bokeh_bokeh-time-inline-dup1}{0.82}
\DefMacro{exp-python-bokeh_bokeh-time-unit-and-inline-dup1}{61.49}
\DefMacro{exp-python-bokeh_bokeh-num-vanilla-dup1}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-unit-dup1}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-inline-dup1}{8}
\DefMacro{exp-python-bokeh_bokeh-num-unit-and-inline-dup1}{8,624}
\DefMacro{exp-python-bokeh_bokeh-timept-vanilla-dup1}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-dup1}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-inline-dup1}{0.102}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-and-inline-dup1}{0.007}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-dup1}{-0.001}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-and-inline-dup1}{0.012}
\DefMacro{exp-python-chubin_cheat.sh-time-vanilla-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-vanilla-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-vanilla-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-dup1}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-vanilla-dup1}{0.97}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-vanilla-dup1}{3}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-vanilla-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-dup1}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-geekcomputers_Python-time-vanilla-dup1}{0.17}
\DefMacro{exp-python-geekcomputers_Python-time-unit-dup1}{0.18}
\DefMacro{exp-python-geekcomputers_Python-time-inline-dup1}{0.19}
\DefMacro{exp-python-geekcomputers_Python-time-unit-and-inline-dup1}{0.37}
\DefMacro{exp-python-geekcomputers_Python-num-vanilla-dup1}{1}
\DefMacro{exp-python-geekcomputers_Python-num-unit-dup1}{1}
\DefMacro{exp-python-geekcomputers_Python-num-inline-dup1}{4}
\DefMacro{exp-python-geekcomputers_Python-num-unit-and-inline-dup1}{5}
\DefMacro{exp-python-geekcomputers_Python-timept-vanilla-dup1}{0.170}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-dup1}{0.181}
\DefMacro{exp-python-geekcomputers_Python-timept-inline-dup1}{0.048}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-and-inline-dup1}{0.075}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-dup1}{0.060}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-and-inline-dup1}{1.198}
\DefMacro{exp-python-google-research_bert-time-vanilla-dup1}{2.05}
\DefMacro{exp-python-google-research_bert-time-unit-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-time-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-time-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-num-vanilla-dup1}{15}
\DefMacro{exp-python-google-research_bert-num-unit-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-num-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-num-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-vanilla-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-dup1}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-and-inline-dup1}{ERROR}
\DefMacro{exp-python-joke2k_faker-time-vanilla-dup1}{15.92}
\DefMacro{exp-python-joke2k_faker-time-unit-dup1}{15.93}
\DefMacro{exp-python-joke2k_faker-time-inline-dup1}{0.27}
\DefMacro{exp-python-joke2k_faker-time-unit-and-inline-dup1}{16.20}
\DefMacro{exp-python-joke2k_faker-num-vanilla-dup1}{1,596}
\DefMacro{exp-python-joke2k_faker-num-unit-dup1}{1,596}
\DefMacro{exp-python-joke2k_faker-num-inline-dup1}{4}
\DefMacro{exp-python-joke2k_faker-num-unit-and-inline-dup1}{1,600}
\DefMacro{exp-python-joke2k_faker-timept-vanilla-dup1}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-unit-dup1}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-inline-dup1}{0.067}
\DefMacro{exp-python-joke2k_faker-timept-unit-and-inline-dup1}{0.010}
\DefMacro{exp-python-joke2k_faker-overhead-unit-dup1}{0.001}
\DefMacro{exp-python-joke2k_faker-overhead-unit-and-inline-dup1}{0.018}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-vanilla-dup1}{7.18}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-dup1}{7.25}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-inline-dup1}{0.40}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-and-inline-dup1}{7.65}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-vanilla-dup1}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-dup1}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-inline-dup1}{1}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-and-inline-dup1}{1,287}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-vanilla-dup1}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-dup1}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-inline-dup1}{0.400}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-and-inline-dup1}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-dup1}{0.009}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-and-inline-dup1}{0.065}
\DefMacro{exp-python-numpy_numpy-time-vanilla-dup1}{3.25}
\DefMacro{exp-python-numpy_numpy-time-unit-dup1}{3.26}
\DefMacro{exp-python-numpy_numpy-time-inline-dup1}{0.52}
\DefMacro{exp-python-numpy_numpy-time-unit-and-inline-dup1}{3.79}
\DefMacro{exp-python-numpy_numpy-num-vanilla-dup1}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-unit-dup1}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-inline-dup1}{2}
\DefMacro{exp-python-numpy_numpy-num-unit-and-inline-dup1}{1}
\DefMacro{exp-python-numpy_numpy-timept-vanilla-dup1}{-3.247}
\DefMacro{exp-python-numpy_numpy-timept-unit-dup1}{-3.261}
\DefMacro{exp-python-numpy_numpy-timept-inline-dup1}{0.262}
\DefMacro{exp-python-numpy_numpy-timept-unit-and-inline-dup1}{3.786}
\DefMacro{exp-python-numpy_numpy-overhead-unit-dup1}{0.004}
\DefMacro{exp-python-numpy_numpy-overhead-unit-and-inline-dup1}{0.166}
\DefMacro{exp-python-pandas-dev_pandas-time-vanilla-dup1}{273.26}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-dup1}{273.37}
\DefMacro{exp-python-pandas-dev_pandas-time-inline-dup1}{0.91}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-and-inline-dup1}{274.28}
\DefMacro{exp-python-pandas-dev_pandas-num-vanilla-dup1}{147,305}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-dup1}{147,305}
\DefMacro{exp-python-pandas-dev_pandas-num-inline-dup1}{2}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-and-inline-dup1}{147,307}
\DefMacro{exp-python-pandas-dev_pandas-timept-vanilla-dup1}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-dup1}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-inline-dup1}{0.455}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-and-inline-dup1}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-dup1}{0.000}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-and-inline-dup1}{0.004}
\DefMacro{exp-python-psf_black-time-vanilla-dup1}{7.07}
\DefMacro{exp-python-psf_black-time-unit-dup1}{7.02}
\DefMacro{exp-python-psf_black-time-inline-dup1}{0.27}
\DefMacro{exp-python-psf_black-time-unit-and-inline-dup1}{7.28}
\DefMacro{exp-python-psf_black-num-vanilla-dup1}{236}
\DefMacro{exp-python-psf_black-num-unit-dup1}{236}
\DefMacro{exp-python-psf_black-num-inline-dup1}{1}
\DefMacro{exp-python-psf_black-num-unit-and-inline-dup1}{237}
\DefMacro{exp-python-psf_black-timept-vanilla-dup1}{0.030}
\DefMacro{exp-python-psf_black-timept-unit-dup1}{0.030}
\DefMacro{exp-python-psf_black-timept-inline-dup1}{0.268}
\DefMacro{exp-python-psf_black-timept-unit-and-inline-dup1}{0.031}
\DefMacro{exp-python-psf_black-overhead-unit-dup1}{-0.008}
\DefMacro{exp-python-psf_black-overhead-unit-and-inline-dup1}{0.030}
\DefMacro{exp-python-pypa_pipenv-time-vanilla-dup1}{4.39}
\DefMacro{exp-python-pypa_pipenv-time-unit-dup1}{4.45}
\DefMacro{exp-python-pypa_pipenv-time-inline-dup1}{0.55}
\DefMacro{exp-python-pypa_pipenv-time-unit-and-inline-dup1}{4.99}
\DefMacro{exp-python-pypa_pipenv-num-vanilla-dup1}{106}
\DefMacro{exp-python-pypa_pipenv-num-unit-dup1}{106}
\DefMacro{exp-python-pypa_pipenv-num-inline-dup1}{1}
\DefMacro{exp-python-pypa_pipenv-num-unit-and-inline-dup1}{107}
\DefMacro{exp-python-pypa_pipenv-timept-vanilla-dup1}{0.041}
\DefMacro{exp-python-pypa_pipenv-timept-unit-dup1}{0.042}
\DefMacro{exp-python-pypa_pipenv-timept-inline-dup1}{0.547}
\DefMacro{exp-python-pypa_pipenv-timept-unit-and-inline-dup1}{0.047}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-dup1}{0.014}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-and-inline-dup1}{0.139}
\DefMacro{exp-python-scrapy_scrapy-time-vanilla-dup1}{2.24}
\DefMacro{exp-python-scrapy_scrapy-time-unit-dup1}{2.36}
\DefMacro{exp-python-scrapy_scrapy-time-inline-dup1}{0.50}
\DefMacro{exp-python-scrapy_scrapy-time-unit-and-inline-dup1}{2.86}
\DefMacro{exp-python-scrapy_scrapy-num-vanilla-dup1}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-unit-dup1}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-inline-dup1}{2}
\DefMacro{exp-python-scrapy_scrapy-num-unit-and-inline-dup1}{1}
\DefMacro{exp-python-scrapy_scrapy-timept-vanilla-dup1}{-2.238}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-dup1}{-2.356}
\DefMacro{exp-python-scrapy_scrapy-timept-inline-dup1}{0.251}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-and-inline-dup1}{2.858}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-dup1}{0.053}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-and-inline-dup1}{0.277}
\DefMacro{exp-python-time-vanilla-AVG-dup1}{59.91}
\DefMacro{exp-python-time-vanilla-SUM-dup1}{599.09}
\DefMacro{exp-python-time-vanilla-MAX-dup1}{273.26}
\DefMacro{exp-python-time-vanilla-MIN-dup1}{0.17}
\DefMacro{exp-python-time-vanilla-MEDIAN-dup1}{7.13}
\DefMacro{exp-python-time-vanilla-STDEV-dup1}{96.66}
\DefMacro{exp-python-time-vanilla-CNT-dup1}{10}
\DefMacro{exp-python-time-unit-AVG-dup1}{60.12}
\DefMacro{exp-python-time-unit-SUM-dup1}{601.22}
\DefMacro{exp-python-time-unit-MAX-dup1}{273.37}
\DefMacro{exp-python-time-unit-MIN-dup1}{0.18}
\DefMacro{exp-python-time-unit-MEDIAN-dup1}{7.13}
\DefMacro{exp-python-time-unit-STDEV-dup1}{96.99}
\DefMacro{exp-python-time-unit-CNT-dup1}{10}
\DefMacro{exp-python-time-inline-AVG-dup1}{0.50}
\DefMacro{exp-python-time-inline-SUM-dup1}{4.97}
\DefMacro{exp-python-time-inline-MAX-dup1}{0.91}
\DefMacro{exp-python-time-inline-MIN-dup1}{0.19}
\DefMacro{exp-python-time-inline-MEDIAN-dup1}{0.51}
\DefMacro{exp-python-time-inline-STDEV-dup1}{0.22}
\DefMacro{exp-python-time-inline-CNT-dup1}{10}
\DefMacro{exp-python-time-unit-and-inline-AVG-dup1}{60.62}
\DefMacro{exp-python-time-unit-and-inline-SUM-dup1}{606.19}
\DefMacro{exp-python-time-unit-and-inline-MAX-dup1}{274.28}
\DefMacro{exp-python-time-unit-and-inline-MIN-dup1}{0.37}
\DefMacro{exp-python-time-unit-and-inline-MEDIAN-dup1}{7.46}
\DefMacro{exp-python-time-unit-and-inline-STDEV-dup1}{97.13}
\DefMacro{exp-python-time-unit-and-inline-CNT-dup1}{10}
\DefMacro{exp-python-num-vanilla-AVG-dup1}{16,011.10}
\DefMacro{exp-python-num-vanilla-SUM-dup1}{160,111}
\DefMacro{exp-python-num-vanilla-MAX-dup1}{147,305}
\DefMacro{exp-python-num-vanilla-MIN-dup1}{-1}
\DefMacro{exp-python-num-vanilla-MEDIAN-dup1}{601.50}
\DefMacro{exp-python-num-vanilla-STDEV-dup1}{43,834.52}
\DefMacro{exp-python-num-vanilla-CNT-dup1}{10}
\DefMacro{exp-python-num-unit-AVG-dup1}{16,011.10}
\DefMacro{exp-python-num-unit-SUM-dup1}{160,111}
\DefMacro{exp-python-num-unit-MAX-dup1}{147,305}
\DefMacro{exp-python-num-unit-MIN-dup1}{-1}
\DefMacro{exp-python-num-unit-MEDIAN-dup1}{601.50}
\DefMacro{exp-python-num-unit-STDEV-dup1}{43,834.52}
\DefMacro{exp-python-num-unit-CNT-dup1}{10}
\DefMacro{exp-python-num-inline-AVG-dup1}{2.70}
\DefMacro{exp-python-num-inline-SUM-dup1}{27}
\DefMacro{exp-python-num-inline-MAX-dup1}{8}
\DefMacro{exp-python-num-inline-MIN-dup1}{1}
\DefMacro{exp-python-num-inline-MEDIAN-dup1}{2.00}
\DefMacro{exp-python-num-inline-STDEV-dup1}{2.05}
\DefMacro{exp-python-num-inline-CNT-dup1}{10}
\DefMacro{exp-python-num-unit-and-inline-AVG-dup1}{16,013.80}
\DefMacro{exp-python-num-unit-and-inline-SUM-dup1}{160,138}
\DefMacro{exp-python-num-unit-and-inline-MAX-dup1}{147,307}
\DefMacro{exp-python-num-unit-and-inline-MIN-dup1}{1}
\DefMacro{exp-python-num-unit-and-inline-MEDIAN-dup1}{603.00}
\DefMacro{exp-python-num-unit-and-inline-STDEV-dup1}{43,834.38}
\DefMacro{exp-python-num-unit-and-inline-CNT-dup1}{10}
\DefMacro{exp-python-timept-vanilla-AVG-dup1}{-0.499}
\DefMacro{exp-python-timept-vanilla-SUM-dup1}{-4.987}
\DefMacro{exp-python-timept-vanilla-MAX-dup1}{0.233}
\DefMacro{exp-python-timept-vanilla-MIN-dup1}{-3.247}
\DefMacro{exp-python-timept-vanilla-MEDIAN-dup1}{0.009}
\DefMacro{exp-python-timept-vanilla-STDEV-dup1}{1.147}
\DefMacro{exp-python-timept-vanilla-CNT-dup1}{10}
\DefMacro{exp-python-timept-unit-AVG-dup1}{-0.511}
\DefMacro{exp-python-timept-unit-SUM-dup1}{-5.107}
\DefMacro{exp-python-timept-unit-MAX-dup1}{0.234}
\DefMacro{exp-python-timept-unit-MIN-dup1}{-3.261}
\DefMacro{exp-python-timept-unit-MEDIAN-dup1}{0.009}
\DefMacro{exp-python-timept-unit-STDEV-dup1}{1.169}
\DefMacro{exp-python-timept-unit-CNT-dup1}{10}
\DefMacro{exp-python-timept-inline-AVG-dup1}{0.267}
\DefMacro{exp-python-timept-inline-SUM-dup1}{2.667}
\DefMacro{exp-python-timept-inline-MAX-dup1}{0.547}
\DefMacro{exp-python-timept-inline-MIN-dup1}{0.048}
\DefMacro{exp-python-timept-inline-MEDIAN-dup1}{0.264}
\DefMacro{exp-python-timept-inline-STDEV-dup1}{0.157}
\DefMacro{exp-python-timept-inline-CNT-dup1}{10}
\DefMacro{exp-python-timept-unit-and-inline-AVG-dup1}{0.706}
\DefMacro{exp-python-timept-unit-and-inline-SUM-dup1}{7.056}
\DefMacro{exp-python-timept-unit-and-inline-MAX-dup1}{3.786}
\DefMacro{exp-python-timept-unit-and-inline-MIN-dup1}{0.002}
\DefMacro{exp-python-timept-unit-and-inline-MEDIAN-dup1}{0.039}
\DefMacro{exp-python-timept-unit-and-inline-STDEV-dup1}{1.326}
\DefMacro{exp-python-timept-unit-and-inline-CNT-dup1}{10}
\DefMacro{exp-python-overhead-unit-AVG-dup1}{0.014}
\DefMacro{exp-python-overhead-unit-SUM-dup1}{0.140}
\DefMacro{exp-python-overhead-unit-MAX-dup1}{0.060}
\DefMacro{exp-python-overhead-unit-MIN-dup1}{-0.008}
\DefMacro{exp-python-overhead-unit-MEDIAN-dup1}{0.006}
\DefMacro{exp-python-overhead-unit-STDEV-dup1}{0.022}
\DefMacro{exp-python-overhead-unit-CNT-dup1}{10}
\DefMacro{exp-python-overhead-unit-and-inline-AVG-dup1}{0.192}
\DefMacro{exp-python-overhead-unit-and-inline-SUM-dup1}{1.919}
\DefMacro{exp-python-overhead-unit-and-inline-MAX-dup1}{1.198}
\DefMacro{exp-python-overhead-unit-and-inline-MIN-dup1}{0.004}
\DefMacro{exp-python-overhead-unit-and-inline-MEDIAN-dup1}{0.047}
\DefMacro{exp-python-overhead-unit-and-inline-STDEV-dup1}{0.346}
\DefMacro{exp-python-overhead-unit-and-inline-CNT-dup1}{10}
\DefMacro{exp-python-timept-vanilla-MACROAVG-dup1}{0.004}
\DefMacro{exp-python-timept-unit-MACROAVG-dup1}{0.004}
\DefMacro{exp-python-timept-inline-MACROAVG-dup1}{0.184}
\DefMacro{exp-python-timept-unit-and-inline-MACROAVG-dup1}{0.004}
\DefMacro{exp-python-overhead-unit-MACROAVG-dup1}{0.004}
\DefMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1}{0.012}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-vanilla-dup10}{224.62}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-dup10}{227.79}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-inline-dup10}{0.56}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-and-inline-dup10}{228.35}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-vanilla-dup10}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-dup10}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-inline-dup10}{20}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-and-inline-dup10}{987}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-vanilla-dup10}{0.232}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-dup10}{0.236}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-inline-dup10}{0.028}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-and-inline-dup10}{0.231}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-dup10}{0.014}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-and-inline-dup10}{0.017}
\DefMacro{exp-python-Textualize_rich-time-vanilla-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-vanilla-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-vanilla-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-dup10}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-bokeh_bokeh-time-vanilla-dup10}{62.41}
\DefMacro{exp-python-bokeh_bokeh-time-unit-dup10}{60.64}
\DefMacro{exp-python-bokeh_bokeh-time-inline-dup10}{0.92}
\DefMacro{exp-python-bokeh_bokeh-time-unit-and-inline-dup10}{61.56}
\DefMacro{exp-python-bokeh_bokeh-num-vanilla-dup10}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-unit-dup10}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-inline-dup10}{80}
\DefMacro{exp-python-bokeh_bokeh-num-unit-and-inline-dup10}{8,696}
\DefMacro{exp-python-bokeh_bokeh-timept-vanilla-dup10}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-dup10}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-inline-dup10}{0.012}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-and-inline-dup10}{0.007}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-dup10}{-0.028}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-and-inline-dup10}{-0.014}
\DefMacro{exp-python-chubin_cheat.sh-time-vanilla-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-vanilla-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-vanilla-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-dup10}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-vanilla-dup10}{0.97}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-vanilla-dup10}{3}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-vanilla-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-dup10}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-geekcomputers_Python-time-vanilla-dup10}{0.17}
\DefMacro{exp-python-geekcomputers_Python-time-unit-dup10}{0.18}
\DefMacro{exp-python-geekcomputers_Python-time-inline-dup10}{0.22}
\DefMacro{exp-python-geekcomputers_Python-time-unit-and-inline-dup10}{0.40}
\DefMacro{exp-python-geekcomputers_Python-num-vanilla-dup10}{1}
\DefMacro{exp-python-geekcomputers_Python-num-unit-dup10}{1}
\DefMacro{exp-python-geekcomputers_Python-num-inline-dup10}{40}
\DefMacro{exp-python-geekcomputers_Python-num-unit-and-inline-dup10}{41}
\DefMacro{exp-python-geekcomputers_Python-timept-vanilla-dup10}{0.173}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-dup10}{0.180}
\DefMacro{exp-python-geekcomputers_Python-timept-inline-dup10}{0.006}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-and-inline-dup10}{0.010}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-dup10}{0.040}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-and-inline-dup10}{1.315}
\DefMacro{exp-python-google-research_bert-time-vanilla-dup10}{2.05}
\DefMacro{exp-python-google-research_bert-time-unit-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-time-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-time-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-num-vanilla-dup10}{15}
\DefMacro{exp-python-google-research_bert-num-unit-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-num-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-num-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-vanilla-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-dup10}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-and-inline-dup10}{ERROR}
\DefMacro{exp-python-joke2k_faker-time-vanilla-dup10}{15.90}
\DefMacro{exp-python-joke2k_faker-time-unit-dup10}{15.95}
\DefMacro{exp-python-joke2k_faker-time-inline-dup10}{0.30}
\DefMacro{exp-python-joke2k_faker-time-unit-and-inline-dup10}{16.24}
\DefMacro{exp-python-joke2k_faker-num-vanilla-dup10}{1,596}
\DefMacro{exp-python-joke2k_faker-num-unit-dup10}{1,596}
\DefMacro{exp-python-joke2k_faker-num-inline-dup10}{40}
\DefMacro{exp-python-joke2k_faker-num-unit-and-inline-dup10}{1,636}
\DefMacro{exp-python-joke2k_faker-timept-vanilla-dup10}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-unit-dup10}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-inline-dup10}{0.007}
\DefMacro{exp-python-joke2k_faker-timept-unit-and-inline-dup10}{0.010}
\DefMacro{exp-python-joke2k_faker-overhead-unit-dup10}{0.003}
\DefMacro{exp-python-joke2k_faker-overhead-unit-and-inline-dup10}{0.022}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-vanilla-dup10}{7.26}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-dup10}{7.24}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-inline-dup10}{0.41}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-and-inline-dup10}{7.65}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-vanilla-dup10}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-dup10}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-inline-dup10}{10}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-and-inline-dup10}{1,296}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-vanilla-dup10}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-dup10}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-inline-dup10}{0.041}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-and-inline-dup10}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-dup10}{-0.002}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-and-inline-dup10}{0.054}
\DefMacro{exp-python-numpy_numpy-time-vanilla-dup10}{3.27}
\DefMacro{exp-python-numpy_numpy-time-unit-dup10}{3.29}
\DefMacro{exp-python-numpy_numpy-time-inline-dup10}{0.54}
\DefMacro{exp-python-numpy_numpy-time-unit-and-inline-dup10}{3.83}
\DefMacro{exp-python-numpy_numpy-num-vanilla-dup10}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-unit-dup10}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-inline-dup10}{20}
\DefMacro{exp-python-numpy_numpy-num-unit-and-inline-dup10}{19}
\DefMacro{exp-python-numpy_numpy-timept-vanilla-dup10}{-3.273}
\DefMacro{exp-python-numpy_numpy-timept-unit-dup10}{-3.286}
\DefMacro{exp-python-numpy_numpy-timept-inline-dup10}{0.027}
\DefMacro{exp-python-numpy_numpy-timept-unit-and-inline-dup10}{0.202}
\DefMacro{exp-python-numpy_numpy-overhead-unit-dup10}{0.004}
\DefMacro{exp-python-numpy_numpy-overhead-unit-and-inline-dup10}{0.170}
\DefMacro{exp-python-pandas-dev_pandas-time-vanilla-dup10}{276.05}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-dup10}{273.10}
\DefMacro{exp-python-pandas-dev_pandas-time-inline-dup10}{0.92}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-and-inline-dup10}{274.02}
\DefMacro{exp-python-pandas-dev_pandas-num-vanilla-dup10}{147,305}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-dup10}{147,307}
\DefMacro{exp-python-pandas-dev_pandas-num-inline-dup10}{20}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-and-inline-dup10}{147,327}
\DefMacro{exp-python-pandas-dev_pandas-timept-vanilla-dup10}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-dup10}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-inline-dup10}{0.046}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-and-inline-dup10}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-dup10}{-0.011}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-and-inline-dup10}{-0.007}
\DefMacro{exp-python-psf_black-time-vanilla-dup10}{7.00}
\DefMacro{exp-python-psf_black-time-unit-dup10}{7.06}
\DefMacro{exp-python-psf_black-time-inline-dup10}{0.27}
\DefMacro{exp-python-psf_black-time-unit-and-inline-dup10}{7.33}
\DefMacro{exp-python-psf_black-num-vanilla-dup10}{236}
\DefMacro{exp-python-psf_black-num-unit-dup10}{236}
\DefMacro{exp-python-psf_black-num-inline-dup10}{10}
\DefMacro{exp-python-psf_black-num-unit-and-inline-dup10}{246}
\DefMacro{exp-python-psf_black-timept-vanilla-dup10}{0.030}
\DefMacro{exp-python-psf_black-timept-unit-dup10}{0.030}
\DefMacro{exp-python-psf_black-timept-inline-dup10}{0.027}
\DefMacro{exp-python-psf_black-timept-unit-and-inline-dup10}{0.030}
\DefMacro{exp-python-psf_black-overhead-unit-dup10}{0.008}
\DefMacro{exp-python-psf_black-overhead-unit-and-inline-dup10}{0.047}
\DefMacro{exp-python-pypa_pipenv-time-vanilla-dup10}{4.37}
\DefMacro{exp-python-pypa_pipenv-time-unit-dup10}{4.44}
\DefMacro{exp-python-pypa_pipenv-time-inline-dup10}{0.55}
\DefMacro{exp-python-pypa_pipenv-time-unit-and-inline-dup10}{5.00}
\DefMacro{exp-python-pypa_pipenv-num-vanilla-dup10}{106}
\DefMacro{exp-python-pypa_pipenv-num-unit-dup10}{106}
\DefMacro{exp-python-pypa_pipenv-num-inline-dup10}{10}
\DefMacro{exp-python-pypa_pipenv-num-unit-and-inline-dup10}{116}
\DefMacro{exp-python-pypa_pipenv-timept-vanilla-dup10}{0.041}
\DefMacro{exp-python-pypa_pipenv-timept-unit-dup10}{0.042}
\DefMacro{exp-python-pypa_pipenv-timept-inline-dup10}{0.055}
\DefMacro{exp-python-pypa_pipenv-timept-unit-and-inline-dup10}{0.043}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-dup10}{0.018}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-and-inline-dup10}{0.144}
\DefMacro{exp-python-scrapy_scrapy-time-vanilla-dup10}{2.23}
\DefMacro{exp-python-scrapy_scrapy-time-unit-dup10}{2.26}
\DefMacro{exp-python-scrapy_scrapy-time-inline-dup10}{0.55}
\DefMacro{exp-python-scrapy_scrapy-time-unit-and-inline-dup10}{2.81}
\DefMacro{exp-python-scrapy_scrapy-num-vanilla-dup10}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-unit-dup10}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-inline-dup10}{20}
\DefMacro{exp-python-scrapy_scrapy-num-unit-and-inline-dup10}{19}
\DefMacro{exp-python-scrapy_scrapy-timept-vanilla-dup10}{-2.234}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-dup10}{-2.261}
\DefMacro{exp-python-scrapy_scrapy-timept-inline-dup10}{0.027}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-and-inline-dup10}{0.148}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-dup10}{0.012}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-and-inline-dup10}{0.258}
\DefMacro{exp-python-time-vanilla-AVG-dup10}{60.33}
\DefMacro{exp-python-time-vanilla-SUM-dup10}{603.29}
\DefMacro{exp-python-time-vanilla-MAX-dup10}{276.05}
\DefMacro{exp-python-time-vanilla-MIN-dup10}{0.17}
\DefMacro{exp-python-time-vanilla-MEDIAN-dup10}{7.13}
\DefMacro{exp-python-time-vanilla-STDEV-dup10}{97.24}
\DefMacro{exp-python-time-vanilla-CNT-dup10}{10}
\DefMacro{exp-python-time-unit-AVG-dup10}{60.19}
\DefMacro{exp-python-time-unit-SUM-dup10}{601.94}
\DefMacro{exp-python-time-unit-MAX-dup10}{273.10}
\DefMacro{exp-python-time-unit-MIN-dup10}{0.18}
\DefMacro{exp-python-time-unit-MEDIAN-dup10}{7.15}
\DefMacro{exp-python-time-unit-STDEV-dup10}{97.11}
\DefMacro{exp-python-time-unit-CNT-dup10}{10}
\DefMacro{exp-python-time-inline-AVG-dup10}{0.53}
\DefMacro{exp-python-time-inline-SUM-dup10}{5.25}
\DefMacro{exp-python-time-inline-MAX-dup10}{0.92}
\DefMacro{exp-python-time-inline-MIN-dup10}{0.22}
\DefMacro{exp-python-time-inline-MEDIAN-dup10}{0.55}
\DefMacro{exp-python-time-inline-STDEV-dup10}{0.23}
\DefMacro{exp-python-time-inline-CNT-dup10}{10}
\DefMacro{exp-python-time-unit-and-inline-AVG-dup10}{60.72}
\DefMacro{exp-python-time-unit-and-inline-SUM-dup10}{607.20}
\DefMacro{exp-python-time-unit-and-inline-MAX-dup10}{274.02}
\DefMacro{exp-python-time-unit-and-inline-MIN-dup10}{0.40}
\DefMacro{exp-python-time-unit-and-inline-MEDIAN-dup10}{7.49}
\DefMacro{exp-python-time-unit-and-inline-STDEV-dup10}{97.25}
\DefMacro{exp-python-time-unit-and-inline-CNT-dup10}{10}
\DefMacro{exp-python-num-vanilla-AVG-dup10}{16,011.10}
\DefMacro{exp-python-num-vanilla-SUM-dup10}{160,111}
\DefMacro{exp-python-num-vanilla-MAX-dup10}{147,305}
\DefMacro{exp-python-num-vanilla-MIN-dup10}{-1}
\DefMacro{exp-python-num-vanilla-MEDIAN-dup10}{601.50}
\DefMacro{exp-python-num-vanilla-STDEV-dup10}{43,834.52}
\DefMacro{exp-python-num-vanilla-CNT-dup10}{10}
\DefMacro{exp-python-num-unit-AVG-dup10}{16,011.30}
\DefMacro{exp-python-num-unit-SUM-dup10}{160,113}
\DefMacro{exp-python-num-unit-MAX-dup10}{147,307}
\DefMacro{exp-python-num-unit-MIN-dup10}{-1}
\DefMacro{exp-python-num-unit-MEDIAN-dup10}{601.50}
\DefMacro{exp-python-num-unit-STDEV-dup10}{43,835.12}
\DefMacro{exp-python-num-unit-CNT-dup10}{10}
\DefMacro{exp-python-num-inline-AVG-dup10}{27.00}
\DefMacro{exp-python-num-inline-SUM-dup10}{270}
\DefMacro{exp-python-num-inline-MAX-dup10}{80}
\DefMacro{exp-python-num-inline-MIN-dup10}{10}
\DefMacro{exp-python-num-inline-MEDIAN-dup10}{20.00}
\DefMacro{exp-python-num-inline-STDEV-dup10}{20.52}
\DefMacro{exp-python-num-inline-CNT-dup10}{10}
\DefMacro{exp-python-num-unit-and-inline-AVG-dup10}{16,038.30}
\DefMacro{exp-python-num-unit-and-inline-SUM-dup10}{160,383}
\DefMacro{exp-python-num-unit-and-inline-MAX-dup10}{147,327}
\DefMacro{exp-python-num-unit-and-inline-MIN-dup10}{19}
\DefMacro{exp-python-num-unit-and-inline-MEDIAN-dup10}{616.50}
\DefMacro{exp-python-num-unit-and-inline-STDEV-dup10}{43,833.78}
\DefMacro{exp-python-num-unit-and-inline-CNT-dup10}{10}
\DefMacro{exp-python-timept-vanilla-AVG-dup10}{-0.501}
\DefMacro{exp-python-timept-vanilla-SUM-dup10}{-5.006}
\DefMacro{exp-python-timept-vanilla-MAX-dup10}{0.232}
\DefMacro{exp-python-timept-vanilla-MIN-dup10}{-3.273}
\DefMacro{exp-python-timept-vanilla-MEDIAN-dup10}{0.009}
\DefMacro{exp-python-timept-vanilla-STDEV-dup10}{1.153}
\DefMacro{exp-python-timept-vanilla-CNT-dup10}{10}
\DefMacro{exp-python-timept-unit-AVG-dup10}{-0.503}
\DefMacro{exp-python-timept-unit-SUM-dup10}{-5.035}
\DefMacro{exp-python-timept-unit-MAX-dup10}{0.236}
\DefMacro{exp-python-timept-unit-MIN-dup10}{-3.286}
\DefMacro{exp-python-timept-unit-MEDIAN-dup10}{0.009}
\DefMacro{exp-python-timept-unit-STDEV-dup10}{1.160}
\DefMacro{exp-python-timept-unit-CNT-dup10}{10}
\DefMacro{exp-python-timept-inline-AVG-dup10}{0.028}
\DefMacro{exp-python-timept-inline-SUM-dup10}{0.277}
\DefMacro{exp-python-timept-inline-MAX-dup10}{0.055}
\DefMacro{exp-python-timept-inline-MIN-dup10}{0.006}
\DefMacro{exp-python-timept-inline-MEDIAN-dup10}{0.027}
\DefMacro{exp-python-timept-inline-STDEV-dup10}{0.016}
\DefMacro{exp-python-timept-inline-CNT-dup10}{10}
\DefMacro{exp-python-timept-unit-and-inline-AVG-dup10}{0.069}
\DefMacro{exp-python-timept-unit-and-inline-SUM-dup10}{0.688}
\DefMacro{exp-python-timept-unit-and-inline-MAX-dup10}{0.231}
\DefMacro{exp-python-timept-unit-and-inline-MIN-dup10}{0.002}
\DefMacro{exp-python-timept-unit-and-inline-MEDIAN-dup10}{0.020}
\DefMacro{exp-python-timept-unit-and-inline-STDEV-dup10}{0.085}
\DefMacro{exp-python-timept-unit-and-inline-CNT-dup10}{10}
\DefMacro{exp-python-overhead-unit-AVG-dup10}{0.006}
\DefMacro{exp-python-overhead-unit-SUM-dup10}{0.057}
\DefMacro{exp-python-overhead-unit-MAX-dup10}{0.040}
\DefMacro{exp-python-overhead-unit-MIN-dup10}{-0.028}
\DefMacro{exp-python-overhead-unit-MEDIAN-dup10}{0.006}
\DefMacro{exp-python-overhead-unit-STDEV-dup10}{0.017}
\DefMacro{exp-python-overhead-unit-CNT-dup10}{10}
\DefMacro{exp-python-overhead-unit-and-inline-AVG-dup10}{0.200}
\DefMacro{exp-python-overhead-unit-and-inline-SUM-dup10}{2.005}
\DefMacro{exp-python-overhead-unit-and-inline-MAX-dup10}{1.315}
\DefMacro{exp-python-overhead-unit-and-inline-MIN-dup10}{-0.014}
\DefMacro{exp-python-overhead-unit-and-inline-MEDIAN-dup10}{0.050}
\DefMacro{exp-python-overhead-unit-and-inline-STDEV-dup10}{0.381}
\DefMacro{exp-python-overhead-unit-and-inline-CNT-dup10}{10}
\DefMacro{exp-python-timept-vanilla-MACROAVG-dup10}{0.004}
\DefMacro{exp-python-timept-unit-MACROAVG-dup10}{0.004}
\DefMacro{exp-python-timept-inline-MACROAVG-dup10}{0.019}
\DefMacro{exp-python-timept-unit-and-inline-MACROAVG-dup10}{0.004}
\DefMacro{exp-python-overhead-unit-MACROAVG-dup10}{-0.002}
\DefMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup10}{0.006}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-vanilla-dup100}{217.25}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-dup100}{255.36}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-inline-dup100}{0.71}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-and-inline-dup100}{256.07}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-vanilla-dup100}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-dup100}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-inline-dup100}{200}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-and-inline-dup100}{1,167}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-vanilla-dup100}{0.225}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-dup100}{0.264}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-inline-dup100}{0.004}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-and-inline-dup100}{0.219}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-dup100}{0.175}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-and-inline-dup100}{0.179}
\DefMacro{exp-python-Textualize_rich-time-vanilla-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-vanilla-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-vanilla-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-dup100}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-bokeh_bokeh-time-vanilla-dup100}{62.24}
\DefMacro{exp-python-bokeh_bokeh-time-unit-dup100}{61.72}
\DefMacro{exp-python-bokeh_bokeh-time-inline-dup100}{1.76}
\DefMacro{exp-python-bokeh_bokeh-time-unit-and-inline-dup100}{63.48}
\DefMacro{exp-python-bokeh_bokeh-num-vanilla-dup100}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-unit-dup100}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-inline-dup100}{800}
\DefMacro{exp-python-bokeh_bokeh-num-unit-and-inline-dup100}{9,416}
\DefMacro{exp-python-bokeh_bokeh-timept-vanilla-dup100}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-dup100}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-inline-dup100}{0.002}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-and-inline-dup100}{0.007}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-dup100}{-0.008}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-and-inline-dup100}{0.020}
\DefMacro{exp-python-chubin_cheat.sh-time-vanilla-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-vanilla-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-vanilla-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-dup100}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-vanilla-dup100}{0.97}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-vanilla-dup100}{3}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-vanilla-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-dup100}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-geekcomputers_Python-time-vanilla-dup100}{0.17}
\DefMacro{exp-python-geekcomputers_Python-time-unit-dup100}{0.18}
\DefMacro{exp-python-geekcomputers_Python-time-inline-dup100}{0.51}
\DefMacro{exp-python-geekcomputers_Python-time-unit-and-inline-dup100}{0.69}
\DefMacro{exp-python-geekcomputers_Python-num-vanilla-dup100}{1}
\DefMacro{exp-python-geekcomputers_Python-num-unit-dup100}{1}
\DefMacro{exp-python-geekcomputers_Python-num-inline-dup100}{400}
\DefMacro{exp-python-geekcomputers_Python-num-unit-and-inline-dup100}{401}
\DefMacro{exp-python-geekcomputers_Python-timept-vanilla-dup100}{0.171}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-dup100}{0.181}
\DefMacro{exp-python-geekcomputers_Python-timept-inline-dup100}{0.001}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-and-inline-dup100}{0.002}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-dup100}{0.059}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-and-inline-dup100}{3.056}
\DefMacro{exp-python-google-research_bert-time-vanilla-dup100}{2.05}
\DefMacro{exp-python-google-research_bert-time-unit-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-time-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-time-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-num-vanilla-dup100}{15}
\DefMacro{exp-python-google-research_bert-num-unit-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-num-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-num-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-vanilla-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-dup100}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-and-inline-dup100}{ERROR}
\DefMacro{exp-python-joke2k_faker-time-vanilla-dup100}{15.90}
\DefMacro{exp-python-joke2k_faker-time-unit-dup100}{15.98}
\DefMacro{exp-python-joke2k_faker-time-inline-dup100}{0.60}
\DefMacro{exp-python-joke2k_faker-time-unit-and-inline-dup100}{16.58}
\DefMacro{exp-python-joke2k_faker-num-vanilla-dup100}{1,596}
\DefMacro{exp-python-joke2k_faker-num-unit-dup100}{1,596}
\DefMacro{exp-python-joke2k_faker-num-inline-dup100}{400}
\DefMacro{exp-python-joke2k_faker-num-unit-and-inline-dup100}{1,996}
\DefMacro{exp-python-joke2k_faker-timept-vanilla-dup100}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-unit-dup100}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-inline-dup100}{0.002}
\DefMacro{exp-python-joke2k_faker-timept-unit-and-inline-dup100}{0.008}
\DefMacro{exp-python-joke2k_faker-overhead-unit-dup100}{0.005}
\DefMacro{exp-python-joke2k_faker-overhead-unit-and-inline-dup100}{0.043}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-vanilla-dup100}{7.22}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-dup100}{7.20}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-inline-dup100}{0.47}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-and-inline-dup100}{7.67}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-vanilla-dup100}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-dup100}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-inline-dup100}{100}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-and-inline-dup100}{1,386}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-vanilla-dup100}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-dup100}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-inline-dup100}{0.005}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-and-inline-dup100}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-dup100}{-0.003}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-and-inline-dup100}{0.062}
\DefMacro{exp-python-numpy_numpy-time-vanilla-dup100}{3.27}
\DefMacro{exp-python-numpy_numpy-time-unit-dup100}{3.27}
\DefMacro{exp-python-numpy_numpy-time-inline-dup100}{0.74}
\DefMacro{exp-python-numpy_numpy-time-unit-and-inline-dup100}{4.01}
\DefMacro{exp-python-numpy_numpy-num-vanilla-dup100}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-unit-dup100}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-inline-dup100}{200}
\DefMacro{exp-python-numpy_numpy-num-unit-and-inline-dup100}{199}
\DefMacro{exp-python-numpy_numpy-timept-vanilla-dup100}{-3.272}
\DefMacro{exp-python-numpy_numpy-timept-unit-dup100}{-3.272}
\DefMacro{exp-python-numpy_numpy-timept-inline-dup100}{0.004}
\DefMacro{exp-python-numpy_numpy-timept-unit-and-inline-dup100}{0.020}
\DefMacro{exp-python-numpy_numpy-overhead-unit-dup100}{-0.000}
\DefMacro{exp-python-numpy_numpy-overhead-unit-and-inline-dup100}{0.227}
\DefMacro{exp-python-pandas-dev_pandas-time-vanilla-dup100}{274.21}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-dup100}{273.10}
\DefMacro{exp-python-pandas-dev_pandas-time-inline-dup100}{1.09}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-and-inline-dup100}{274.19}
\DefMacro{exp-python-pandas-dev_pandas-num-vanilla-dup100}{147,306}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-dup100}{147,306}
\DefMacro{exp-python-pandas-dev_pandas-num-inline-dup100}{200}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-and-inline-dup100}{147,506}
\DefMacro{exp-python-pandas-dev_pandas-timept-vanilla-dup100}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-dup100}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-inline-dup100}{0.005}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-and-inline-dup100}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-dup100}{-0.004}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-and-inline-dup100}{-0.000}
\DefMacro{exp-python-psf_black-time-vanilla-dup100}{7.03}
\DefMacro{exp-python-psf_black-time-unit-dup100}{7.07}
\DefMacro{exp-python-psf_black-time-inline-dup100}{0.35}
\DefMacro{exp-python-psf_black-time-unit-and-inline-dup100}{7.42}
\DefMacro{exp-python-psf_black-num-vanilla-dup100}{236}
\DefMacro{exp-python-psf_black-num-unit-dup100}{236}
\DefMacro{exp-python-psf_black-num-inline-dup100}{100}
\DefMacro{exp-python-psf_black-num-unit-and-inline-dup100}{336}
\DefMacro{exp-python-psf_black-timept-vanilla-dup100}{0.030}
\DefMacro{exp-python-psf_black-timept-unit-dup100}{0.030}
\DefMacro{exp-python-psf_black-timept-inline-dup100}{0.004}
\DefMacro{exp-python-psf_black-timept-unit-and-inline-dup100}{0.022}
\DefMacro{exp-python-psf_black-overhead-unit-dup100}{0.005}
\DefMacro{exp-python-psf_black-overhead-unit-and-inline-dup100}{0.055}
\DefMacro{exp-python-pypa_pipenv-time-vanilla-dup100}{4.37}
\DefMacro{exp-python-pypa_pipenv-time-unit-dup100}{4.32}
\DefMacro{exp-python-pypa_pipenv-time-inline-dup100}{0.63}
\DefMacro{exp-python-pypa_pipenv-time-unit-and-inline-dup100}{4.94}
\DefMacro{exp-python-pypa_pipenv-num-vanilla-dup100}{106}
\DefMacro{exp-python-pypa_pipenv-num-unit-dup100}{106}
\DefMacro{exp-python-pypa_pipenv-num-inline-dup100}{100}
\DefMacro{exp-python-pypa_pipenv-num-unit-and-inline-dup100}{206}
\DefMacro{exp-python-pypa_pipenv-timept-vanilla-dup100}{0.041}
\DefMacro{exp-python-pypa_pipenv-timept-unit-dup100}{0.041}
\DefMacro{exp-python-pypa_pipenv-timept-inline-dup100}{0.006}
\DefMacro{exp-python-pypa_pipenv-timept-unit-and-inline-dup100}{0.024}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-dup100}{-0.012}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-and-inline-dup100}{0.132}
\DefMacro{exp-python-scrapy_scrapy-time-vanilla-dup100}{2.28}
\DefMacro{exp-python-scrapy_scrapy-time-unit-dup100}{2.22}
\DefMacro{exp-python-scrapy_scrapy-time-inline-dup100}{0.75}
\DefMacro{exp-python-scrapy_scrapy-time-unit-and-inline-dup100}{2.97}
\DefMacro{exp-python-scrapy_scrapy-num-vanilla-dup100}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-unit-dup100}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-inline-dup100}{200}
\DefMacro{exp-python-scrapy_scrapy-num-unit-and-inline-dup100}{199}
\DefMacro{exp-python-scrapy_scrapy-timept-vanilla-dup100}{-2.285}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-dup100}{-2.220}
\DefMacro{exp-python-scrapy_scrapy-timept-inline-dup100}{0.004}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-and-inline-dup100}{0.015}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-dup100}{-0.028}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-and-inline-dup100}{0.301}
\DefMacro{exp-python-time-vanilla-AVG-dup100}{59.39}
\DefMacro{exp-python-time-vanilla-SUM-dup100}{593.93}
\DefMacro{exp-python-time-vanilla-MAX-dup100}{274.21}
\DefMacro{exp-python-time-vanilla-MIN-dup100}{0.17}
\DefMacro{exp-python-time-vanilla-MEDIAN-dup100}{7.12}
\DefMacro{exp-python-time-vanilla-STDEV-dup100}{95.59}
\DefMacro{exp-python-time-vanilla-CNT-dup100}{10}
\DefMacro{exp-python-time-unit-AVG-dup100}{63.04}
\DefMacro{exp-python-time-unit-SUM-dup100}{630.42}
\DefMacro{exp-python-time-unit-MAX-dup100}{273.10}
\DefMacro{exp-python-time-unit-MIN-dup100}{0.18}
\DefMacro{exp-python-time-unit-MEDIAN-dup100}{7.13}
\DefMacro{exp-python-time-unit-STDEV-dup100}{102.10}
\DefMacro{exp-python-time-unit-CNT-dup100}{10}
\DefMacro{exp-python-time-inline-AVG-dup100}{0.76}
\DefMacro{exp-python-time-inline-SUM-dup100}{7.60}
\DefMacro{exp-python-time-inline-MAX-dup100}{1.76}
\DefMacro{exp-python-time-inline-MIN-dup100}{0.35}
\DefMacro{exp-python-time-inline-MEDIAN-dup100}{0.67}
\DefMacro{exp-python-time-inline-STDEV-dup100}{0.38}
\DefMacro{exp-python-time-inline-CNT-dup100}{10}
\DefMacro{exp-python-time-unit-and-inline-AVG-dup100}{63.80}
\DefMacro{exp-python-time-unit-and-inline-SUM-dup100}{638.02}
\DefMacro{exp-python-time-unit-and-inline-MAX-dup100}{274.19}
\DefMacro{exp-python-time-unit-and-inline-MIN-dup100}{0.69}
\DefMacro{exp-python-time-unit-and-inline-MEDIAN-dup100}{7.54}
\DefMacro{exp-python-time-unit-and-inline-STDEV-dup100}{102.23}
\DefMacro{exp-python-time-unit-and-inline-CNT-dup100}{10}
\DefMacro{exp-python-num-vanilla-AVG-dup100}{16,011.20}
\DefMacro{exp-python-num-vanilla-SUM-dup100}{160,112}
\DefMacro{exp-python-num-vanilla-MAX-dup100}{147,306}
\DefMacro{exp-python-num-vanilla-MIN-dup100}{-1}
\DefMacro{exp-python-num-vanilla-MEDIAN-dup100}{601.50}
\DefMacro{exp-python-num-vanilla-STDEV-dup100}{43,834.82}
\DefMacro{exp-python-num-vanilla-CNT-dup100}{10}
\DefMacro{exp-python-num-unit-AVG-dup100}{16,011.20}
\DefMacro{exp-python-num-unit-SUM-dup100}{160,112}
\DefMacro{exp-python-num-unit-MAX-dup100}{147,306}
\DefMacro{exp-python-num-unit-MIN-dup100}{-1}
\DefMacro{exp-python-num-unit-MEDIAN-dup100}{601.50}
\DefMacro{exp-python-num-unit-STDEV-dup100}{43,834.82}
\DefMacro{exp-python-num-unit-CNT-dup100}{10}
\DefMacro{exp-python-num-inline-AVG-dup100}{270.00}
\DefMacro{exp-python-num-inline-SUM-dup100}{2,700}
\DefMacro{exp-python-num-inline-MAX-dup100}{800}
\DefMacro{exp-python-num-inline-MIN-dup100}{100}
\DefMacro{exp-python-num-inline-MEDIAN-dup100}{200.00}
\DefMacro{exp-python-num-inline-STDEV-dup100}{205.18}
\DefMacro{exp-python-num-inline-CNT-dup100}{10}
\DefMacro{exp-python-num-unit-and-inline-AVG-dup100}{16,281.20}
\DefMacro{exp-python-num-unit-and-inline-SUM-dup100}{162,812}
\DefMacro{exp-python-num-unit-and-inline-MAX-dup100}{147,506}
\DefMacro{exp-python-num-unit-and-inline-MIN-dup100}{199}
\DefMacro{exp-python-num-unit-and-inline-MEDIAN-dup100}{784.00}
\DefMacro{exp-python-num-unit-and-inline-STDEV-dup100}{43,821.88}
\DefMacro{exp-python-num-unit-and-inline-CNT-dup100}{10}
\DefMacro{exp-python-timept-vanilla-AVG-dup100}{-0.507}
\DefMacro{exp-python-timept-vanilla-SUM-dup100}{-5.066}
\DefMacro{exp-python-timept-vanilla-MAX-dup100}{0.225}
\DefMacro{exp-python-timept-vanilla-MIN-dup100}{-3.272}
\DefMacro{exp-python-timept-vanilla-MEDIAN-dup100}{0.009}
\DefMacro{exp-python-timept-vanilla-STDEV-dup100}{1.159}
\DefMacro{exp-python-timept-vanilla-CNT-dup100}{10}
\DefMacro{exp-python-timept-unit-AVG-dup100}{-0.495}
\DefMacro{exp-python-timept-unit-SUM-dup100}{-4.952}
\DefMacro{exp-python-timept-unit-MAX-dup100}{0.264}
\DefMacro{exp-python-timept-unit-MIN-dup100}{-3.272}
\DefMacro{exp-python-timept-unit-MEDIAN-dup100}{0.009}
\DefMacro{exp-python-timept-unit-STDEV-dup100}{1.153}
\DefMacro{exp-python-timept-unit-CNT-dup100}{10}
\DefMacro{exp-python-timept-inline-AVG-dup100}{0.004}
\DefMacro{exp-python-timept-inline-SUM-dup100}{0.036}
\DefMacro{exp-python-timept-inline-MAX-dup100}{0.006}
\DefMacro{exp-python-timept-inline-MIN-dup100}{0.001}
\DefMacro{exp-python-timept-inline-MEDIAN-dup100}{0.004}
\DefMacro{exp-python-timept-inline-STDEV-dup100}{0.002}
\DefMacro{exp-python-timept-inline-CNT-dup100}{10}
\DefMacro{exp-python-timept-unit-and-inline-AVG-dup100}{0.032}
\DefMacro{exp-python-timept-unit-and-inline-SUM-dup100}{0.325}
\DefMacro{exp-python-timept-unit-and-inline-MAX-dup100}{0.219}
\DefMacro{exp-python-timept-unit-and-inline-MIN-dup100}{0.002}
\DefMacro{exp-python-timept-unit-and-inline-MEDIAN-dup100}{0.012}
\DefMacro{exp-python-timept-unit-and-inline-STDEV-dup100}{0.063}
\DefMacro{exp-python-timept-unit-and-inline-CNT-dup100}{10}
\DefMacro{exp-python-overhead-unit-AVG-dup100}{0.019}
\DefMacro{exp-python-overhead-unit-SUM-dup100}{0.191}
\DefMacro{exp-python-overhead-unit-MAX-dup100}{0.175}
\DefMacro{exp-python-overhead-unit-MIN-dup100}{-0.028}
\DefMacro{exp-python-overhead-unit-MEDIAN-dup100}{-0.001}
\DefMacro{exp-python-overhead-unit-STDEV-dup100}{0.056}
\DefMacro{exp-python-overhead-unit-CNT-dup100}{10}
\DefMacro{exp-python-overhead-unit-and-inline-AVG-dup100}{0.407}
\DefMacro{exp-python-overhead-unit-and-inline-SUM-dup100}{4.075}
\DefMacro{exp-python-overhead-unit-and-inline-MAX-dup100}{3.056}
\DefMacro{exp-python-overhead-unit-and-inline-MIN-dup100}{-0.000}
\DefMacro{exp-python-overhead-unit-and-inline-MEDIAN-dup100}{0.097}
\DefMacro{exp-python-overhead-unit-and-inline-STDEV-dup100}{0.888}
\DefMacro{exp-python-overhead-unit-and-inline-CNT-dup100}{10}
\DefMacro{exp-python-timept-vanilla-MACROAVG-dup100}{0.004}
\DefMacro{exp-python-timept-unit-MACROAVG-dup100}{0.004}
\DefMacro{exp-python-timept-inline-MACROAVG-dup100}{0.003}
\DefMacro{exp-python-timept-unit-and-inline-MACROAVG-dup100}{0.004}
\DefMacro{exp-python-overhead-unit-MACROAVG-dup100}{0.061}
\DefMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup100}{0.074}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-vanilla-dup1000}{265.71}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-dup1000}{263.30}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-inline-dup1000}{3.11}
\DefMacro{exp-python-RaRe-Technologies_gensim-time-unit-and-inline-dup1000}{266.41}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-vanilla-dup1000}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-dup1000}{967}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-inline-dup1000}{2,000}
\DefMacro{exp-python-RaRe-Technologies_gensim-num-unit-and-inline-dup1000}{2,967}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-vanilla-dup1000}{0.275}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-dup1000}{0.272}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-RaRe-Technologies_gensim-timept-unit-and-inline-dup1000}{0.090}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-dup1000}{-0.009}
\DefMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-and-inline-dup1000}{0.003}
\DefMacro{exp-python-Textualize_rich-time-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-python-Textualize_rich-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-bokeh_bokeh-time-vanilla-dup1000}{65.11}
\DefMacro{exp-python-bokeh_bokeh-time-unit-dup1000}{62.49}
\DefMacro{exp-python-bokeh_bokeh-time-inline-dup1000}{15.61}
\DefMacro{exp-python-bokeh_bokeh-time-unit-and-inline-dup1000}{78.10}
\DefMacro{exp-python-bokeh_bokeh-num-vanilla-dup1000}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-unit-dup1000}{8,616}
\DefMacro{exp-python-bokeh_bokeh-num-inline-dup1000}{8,000}
\DefMacro{exp-python-bokeh_bokeh-num-unit-and-inline-dup1000}{16,616}
\DefMacro{exp-python-bokeh_bokeh-timept-vanilla-dup1000}{0.008}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-dup1000}{0.007}
\DefMacro{exp-python-bokeh_bokeh-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-bokeh_bokeh-timept-unit-and-inline-dup1000}{0.005}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-dup1000}{-0.040}
\DefMacro{exp-python-bokeh_bokeh-overhead-unit-and-inline-dup1000}{0.200}
\DefMacro{exp-python-chubin_cheat.sh-time-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-python-chubin_cheat.sh-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-vanilla-dup1000}{0.97}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-vanilla-dup1000}{3}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-python-davidsandberg_facenet-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-geekcomputers_Python-time-vanilla-dup1000}{0.17}
\DefMacro{exp-python-geekcomputers_Python-time-unit-dup1000}{0.20}
\DefMacro{exp-python-geekcomputers_Python-time-inline-dup1000}{5.68}
\DefMacro{exp-python-geekcomputers_Python-time-unit-and-inline-dup1000}{5.88}
\DefMacro{exp-python-geekcomputers_Python-num-vanilla-dup1000}{1}
\DefMacro{exp-python-geekcomputers_Python-num-unit-dup1000}{1}
\DefMacro{exp-python-geekcomputers_Python-num-inline-dup1000}{4,000}
\DefMacro{exp-python-geekcomputers_Python-num-unit-and-inline-dup1000}{4,001}
\DefMacro{exp-python-geekcomputers_Python-timept-vanilla-dup1000}{0.171}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-dup1000}{0.198}
\DefMacro{exp-python-geekcomputers_Python-timept-inline-dup1000}{0.001}
\DefMacro{exp-python-geekcomputers_Python-timept-unit-and-inline-dup1000}{0.001}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-dup1000}{0.159}
\DefMacro{exp-python-geekcomputers_Python-overhead-unit-and-inline-dup1000}{33.402}
\DefMacro{exp-python-google-research_bert-time-vanilla-dup1000}{2.05}
\DefMacro{exp-python-google-research_bert-time-unit-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-time-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-time-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-num-vanilla-dup1000}{15}
\DefMacro{exp-python-google-research_bert-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-num-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-num-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-timept-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-dup1000}{ERROR}
\DefMacro{exp-python-google-research_bert-overhead-unit-and-inline-dup1000}{ERROR}
\DefMacro{exp-python-joke2k_faker-time-vanilla-dup1000}{15.91}
\DefMacro{exp-python-joke2k_faker-time-unit-dup1000}{16.94}
\DefMacro{exp-python-joke2k_faker-time-inline-dup1000}{5.45}
\DefMacro{exp-python-joke2k_faker-time-unit-and-inline-dup1000}{22.39}
\DefMacro{exp-python-joke2k_faker-num-vanilla-dup1000}{1,596}
\DefMacro{exp-python-joke2k_faker-num-unit-dup1000}{1,596}
\DefMacro{exp-python-joke2k_faker-num-inline-dup1000}{4,000}
\DefMacro{exp-python-joke2k_faker-num-unit-and-inline-dup1000}{5,596}
\DefMacro{exp-python-joke2k_faker-timept-vanilla-dup1000}{0.010}
\DefMacro{exp-python-joke2k_faker-timept-unit-dup1000}{0.011}
\DefMacro{exp-python-joke2k_faker-timept-inline-dup1000}{0.001}
\DefMacro{exp-python-joke2k_faker-timept-unit-and-inline-dup1000}{0.004}
\DefMacro{exp-python-joke2k_faker-overhead-unit-dup1000}{0.065}
\DefMacro{exp-python-joke2k_faker-overhead-unit-and-inline-dup1000}{0.407}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-vanilla-dup1000}{7.23}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-dup1000}{7.38}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-inline-dup1000}{1.60}
\DefMacro{exp-python-mitmproxy_mitmproxy-time-unit-and-inline-dup1000}{8.98}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-vanilla-dup1000}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-dup1000}{1,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-inline-dup1000}{1,000}
\DefMacro{exp-python-mitmproxy_mitmproxy-num-unit-and-inline-dup1000}{2,286}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-vanilla-dup1000}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-dup1000}{0.006}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-mitmproxy_mitmproxy-timept-unit-and-inline-dup1000}{0.004}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-dup1000}{0.020}
\DefMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-and-inline-dup1000}{0.241}
\DefMacro{exp-python-numpy_numpy-time-vanilla-dup1000}{3.27}
\DefMacro{exp-python-numpy_numpy-time-unit-dup1000}{3.28}
\DefMacro{exp-python-numpy_numpy-time-inline-dup1000}{3.35}
\DefMacro{exp-python-numpy_numpy-time-unit-and-inline-dup1000}{6.63}
\DefMacro{exp-python-numpy_numpy-num-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-numpy_numpy-num-inline-dup1000}{2,000}
\DefMacro{exp-python-numpy_numpy-num-unit-and-inline-dup1000}{1,999}
\DefMacro{exp-python-numpy_numpy-timept-vanilla-dup1000}{-3.275}
\DefMacro{exp-python-numpy_numpy-timept-unit-dup1000}{-3.282}
\DefMacro{exp-python-numpy_numpy-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-numpy_numpy-timept-unit-and-inline-dup1000}{0.003}
\DefMacro{exp-python-numpy_numpy-overhead-unit-dup1000}{0.002}
\DefMacro{exp-python-numpy_numpy-overhead-unit-and-inline-dup1000}{1.025}
\DefMacro{exp-python-pandas-dev_pandas-time-vanilla-dup1000}{278.23}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-dup1000}{273.16}
\DefMacro{exp-python-pandas-dev_pandas-time-inline-dup1000}{3.61}
\DefMacro{exp-python-pandas-dev_pandas-time-unit-and-inline-dup1000}{276.77}
\DefMacro{exp-python-pandas-dev_pandas-num-vanilla-dup1000}{147,307}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-dup1000}{147,306}
\DefMacro{exp-python-pandas-dev_pandas-num-inline-dup1000}{2,000}
\DefMacro{exp-python-pandas-dev_pandas-num-unit-and-inline-dup1000}{149,306}
\DefMacro{exp-python-pandas-dev_pandas-timept-vanilla-dup1000}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-dup1000}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-timept-unit-and-inline-dup1000}{0.002}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-dup1000}{-0.018}
\DefMacro{exp-python-pandas-dev_pandas-overhead-unit-and-inline-dup1000}{-0.005}
\DefMacro{exp-python-psf_black-time-vanilla-dup1000}{7.02}
\DefMacro{exp-python-psf_black-time-unit-dup1000}{7.37}
\DefMacro{exp-python-psf_black-time-inline-dup1000}{1.59}
\DefMacro{exp-python-psf_black-time-unit-and-inline-dup1000}{8.96}
\DefMacro{exp-python-psf_black-num-vanilla-dup1000}{236}
\DefMacro{exp-python-psf_black-num-unit-dup1000}{236}
\DefMacro{exp-python-psf_black-num-inline-dup1000}{1,000}
\DefMacro{exp-python-psf_black-num-unit-and-inline-dup1000}{1,236}
\DefMacro{exp-python-psf_black-timept-vanilla-dup1000}{0.030}
\DefMacro{exp-python-psf_black-timept-unit-dup1000}{0.031}
\DefMacro{exp-python-psf_black-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-psf_black-timept-unit-and-inline-dup1000}{0.007}
\DefMacro{exp-python-psf_black-overhead-unit-dup1000}{0.050}
\DefMacro{exp-python-psf_black-overhead-unit-and-inline-dup1000}{0.276}
\DefMacro{exp-python-pypa_pipenv-time-vanilla-dup1000}{4.62}
\DefMacro{exp-python-pypa_pipenv-time-unit-dup1000}{4.49}
\DefMacro{exp-python-pypa_pipenv-time-inline-dup1000}{1.77}
\DefMacro{exp-python-pypa_pipenv-time-unit-and-inline-dup1000}{6.26}
\DefMacro{exp-python-pypa_pipenv-num-vanilla-dup1000}{106}
\DefMacro{exp-python-pypa_pipenv-num-unit-dup1000}{106}
\DefMacro{exp-python-pypa_pipenv-num-inline-dup1000}{1,000}
\DefMacro{exp-python-pypa_pipenv-num-unit-and-inline-dup1000}{1,106}
\DefMacro{exp-python-pypa_pipenv-timept-vanilla-dup1000}{0.044}
\DefMacro{exp-python-pypa_pipenv-timept-unit-dup1000}{0.042}
\DefMacro{exp-python-pypa_pipenv-timept-inline-dup1000}{0.002}
\DefMacro{exp-python-pypa_pipenv-timept-unit-and-inline-dup1000}{0.006}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-dup1000}{-0.029}
\DefMacro{exp-python-pypa_pipenv-overhead-unit-and-inline-dup1000}{0.353}
\DefMacro{exp-python-scrapy_scrapy-time-vanilla-dup1000}{2.25}
\DefMacro{exp-python-scrapy_scrapy-time-unit-dup1000}{2.34}
\DefMacro{exp-python-scrapy_scrapy-time-inline-dup1000}{6.81}
\DefMacro{exp-python-scrapy_scrapy-time-unit-and-inline-dup1000}{9.14}
\DefMacro{exp-python-scrapy_scrapy-num-vanilla-dup1000}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-unit-dup1000}{ERROR}
\DefMacro{exp-python-scrapy_scrapy-num-inline-dup1000}{2,000}
\DefMacro{exp-python-scrapy_scrapy-num-unit-and-inline-dup1000}{1,999}
\DefMacro{exp-python-scrapy_scrapy-timept-vanilla-dup1000}{-2.252}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-dup1000}{-2.338}
\DefMacro{exp-python-scrapy_scrapy-timept-inline-dup1000}{0.003}
\DefMacro{exp-python-scrapy_scrapy-timept-unit-and-inline-dup1000}{0.005}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-dup1000}{0.038}
\DefMacro{exp-python-scrapy_scrapy-overhead-unit-and-inline-dup1000}{3.061}
\DefMacro{exp-python-time-vanilla-AVG-dup1000}{64.95}
\DefMacro{exp-python-time-vanilla-SUM-dup1000}{649.53}
\DefMacro{exp-python-time-vanilla-MAX-dup1000}{278.23}
\DefMacro{exp-python-time-vanilla-MIN-dup1000}{0.17}
\DefMacro{exp-python-time-vanilla-MEDIAN-dup1000}{7.13}
\DefMacro{exp-python-time-vanilla-STDEV-dup1000}{105.10}
\DefMacro{exp-python-time-vanilla-CNT-dup1000}{10}
\DefMacro{exp-python-time-unit-AVG-dup1000}{64.09}
\DefMacro{exp-python-time-unit-SUM-dup1000}{640.93}
\DefMacro{exp-python-time-unit-MAX-dup1000}{273.16}
\DefMacro{exp-python-time-unit-MIN-dup1000}{0.20}
\DefMacro{exp-python-time-unit-MEDIAN-dup1000}{7.37}
\DefMacro{exp-python-time-unit-STDEV-dup1000}{103.54}
\DefMacro{exp-python-time-unit-CNT-dup1000}{10}
\DefMacro{exp-python-time-inline-AVG-dup1000}{4.86}
\DefMacro{exp-python-time-inline-SUM-dup1000}{48.57}
\DefMacro{exp-python-time-inline-MAX-dup1000}{15.61}
\DefMacro{exp-python-time-inline-MIN-dup1000}{1.59}
\DefMacro{exp-python-time-inline-MEDIAN-dup1000}{3.48}
\DefMacro{exp-python-time-inline-STDEV-dup1000}{3.98}
\DefMacro{exp-python-time-inline-CNT-dup1000}{10}
\DefMacro{exp-python-time-unit-and-inline-AVG-dup1000}{68.95}
\DefMacro{exp-python-time-unit-and-inline-SUM-dup1000}{689.50}
\DefMacro{exp-python-time-unit-and-inline-MAX-dup1000}{276.77}
\DefMacro{exp-python-time-unit-and-inline-MIN-dup1000}{5.88}
\DefMacro{exp-python-time-unit-and-inline-MEDIAN-dup1000}{9.06}
\DefMacro{exp-python-time-unit-and-inline-STDEV-dup1000}{103.44}
\DefMacro{exp-python-time-unit-and-inline-CNT-dup1000}{10}
\DefMacro{exp-python-num-vanilla-AVG-dup1000}{16,011.30}
\DefMacro{exp-python-num-vanilla-SUM-dup1000}{160,113}
\DefMacro{exp-python-num-vanilla-MAX-dup1000}{147,307}
\DefMacro{exp-python-num-vanilla-MIN-dup1000}{-1}
\DefMacro{exp-python-num-vanilla-MEDIAN-dup1000}{601.50}
\DefMacro{exp-python-num-vanilla-STDEV-dup1000}{43,835.12}
\DefMacro{exp-python-num-vanilla-CNT-dup1000}{10}
\DefMacro{exp-python-num-unit-AVG-dup1000}{16,011.20}
\DefMacro{exp-python-num-unit-SUM-dup1000}{160,112}
\DefMacro{exp-python-num-unit-MAX-dup1000}{147,306}
\DefMacro{exp-python-num-unit-MIN-dup1000}{-1}
\DefMacro{exp-python-num-unit-MEDIAN-dup1000}{601.50}
\DefMacro{exp-python-num-unit-STDEV-dup1000}{43,834.82}
\DefMacro{exp-python-num-unit-CNT-dup1000}{10}
\DefMacro{exp-python-num-inline-AVG-dup1000}{2,700.00}
\DefMacro{exp-python-num-inline-SUM-dup1000}{27,000}
\DefMacro{exp-python-num-inline-MAX-dup1000}{8,000}
\DefMacro{exp-python-num-inline-MIN-dup1000}{1,000}
\DefMacro{exp-python-num-inline-MEDIAN-dup1000}{2,000.00}
\DefMacro{exp-python-num-inline-STDEV-dup1000}{2,051.83}
\DefMacro{exp-python-num-inline-CNT-dup1000}{10}
\DefMacro{exp-python-num-unit-and-inline-AVG-dup1000}{18,711.20}
\DefMacro{exp-python-num-unit-and-inline-SUM-dup1000}{187,112}
\DefMacro{exp-python-num-unit-and-inline-MAX-dup1000}{149,306}
\DefMacro{exp-python-num-unit-and-inline-MIN-dup1000}{1,106}
\DefMacro{exp-python-num-unit-and-inline-MEDIAN-dup1000}{2,626.50}
\DefMacro{exp-python-num-unit-and-inline-STDEV-dup1000}{43,748.57}
\DefMacro{exp-python-num-unit-and-inline-CNT-dup1000}{10}
\DefMacro{exp-python-timept-vanilla-AVG-dup1000}{-0.498}
\DefMacro{exp-python-timept-vanilla-SUM-dup1000}{-4.983}
\DefMacro{exp-python-timept-vanilla-MAX-dup1000}{0.275}
\DefMacro{exp-python-timept-vanilla-MIN-dup1000}{-3.275}
\DefMacro{exp-python-timept-vanilla-MEDIAN-dup1000}{0.009}
\DefMacro{exp-python-timept-vanilla-STDEV-dup1000}{1.158}
\DefMacro{exp-python-timept-vanilla-CNT-dup1000}{10}
\DefMacro{exp-python-timept-unit-AVG-dup1000}{-0.505}
\DefMacro{exp-python-timept-unit-SUM-dup1000}{-5.051}
\DefMacro{exp-python-timept-unit-MAX-dup1000}{0.272}
\DefMacro{exp-python-timept-unit-MIN-dup1000}{-3.282}
\DefMacro{exp-python-timept-unit-MEDIAN-dup1000}{0.009}
\DefMacro{exp-python-timept-unit-STDEV-dup1000}{1.175}
\DefMacro{exp-python-timept-unit-CNT-dup1000}{10}
\DefMacro{exp-python-timept-inline-AVG-dup1000}{0.002}
\DefMacro{exp-python-timept-inline-SUM-dup1000}{0.018}
\DefMacro{exp-python-timept-inline-MAX-dup1000}{0.003}
\DefMacro{exp-python-timept-inline-MIN-dup1000}{0.001}
\DefMacro{exp-python-timept-inline-MEDIAN-dup1000}{0.002}
\DefMacro{exp-python-timept-inline-STDEV-dup1000}{0.001}
\DefMacro{exp-python-timept-inline-CNT-dup1000}{10}
\DefMacro{exp-python-timept-unit-and-inline-AVG-dup1000}{0.013}
\DefMacro{exp-python-timept-unit-and-inline-SUM-dup1000}{0.127}
\DefMacro{exp-python-timept-unit-and-inline-MAX-dup1000}{0.090}
\DefMacro{exp-python-timept-unit-and-inline-MIN-dup1000}{0.001}
\DefMacro{exp-python-timept-unit-and-inline-MEDIAN-dup1000}{0.004}
\DefMacro{exp-python-timept-unit-and-inline-STDEV-dup1000}{0.026}
\DefMacro{exp-python-timept-unit-and-inline-CNT-dup1000}{10}
\DefMacro{exp-python-overhead-unit-AVG-dup1000}{0.024}
\DefMacro{exp-python-overhead-unit-SUM-dup1000}{0.237}
\DefMacro{exp-python-overhead-unit-MAX-dup1000}{0.159}
\DefMacro{exp-python-overhead-unit-MIN-dup1000}{-0.040}
\DefMacro{exp-python-overhead-unit-MEDIAN-dup1000}{0.011}
\DefMacro{exp-python-overhead-unit-STDEV-dup1000}{0.056}
\DefMacro{exp-python-overhead-unit-CNT-dup1000}{10}
\DefMacro{exp-python-overhead-unit-and-inline-AVG-dup1000}{3.896}
\DefMacro{exp-python-overhead-unit-and-inline-SUM-dup1000}{38.962}
\DefMacro{exp-python-overhead-unit-and-inline-MAX-dup1000}{33.402}
\DefMacro{exp-python-overhead-unit-and-inline-MIN-dup1000}{-0.005}
\DefMacro{exp-python-overhead-unit-and-inline-MEDIAN-dup1000}{0.314}
\DefMacro{exp-python-overhead-unit-and-inline-STDEV-dup1000}{9.873}
\DefMacro{exp-python-overhead-unit-and-inline-CNT-dup1000}{10}
\DefMacro{exp-python-timept-vanilla-MACROAVG-dup1000}{0.004}
\DefMacro{exp-python-timept-unit-MACROAVG-dup1000}{0.004}
\DefMacro{exp-python-timept-inline-MACROAVG-dup1000}{0.002}
\DefMacro{exp-python-timept-unit-and-inline-MACROAVG-dup1000}{0.004}
\DefMacro{exp-python-overhead-unit-MACROAVG-dup1000}{-0.013}
\DefMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1000}{0.062}

==> tables/data-exp-skips-java.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-java-proj-initial}{37}
\DefMacro{exp-java-skipped}{10}
\DefMacro{exp-java-proj-can-run}{27}
\DefMacro{exp-java-skipped-compilation-failure}{10}
\DefMacro{exp-java-skipped-unit-tests}{20}
\DefMacro{exp-java-proj-can-run-unit-tests}{7}
\DefMacro{exp-java-skipped-unit-tests-too-many-test-failures}{17}
\DefMacro{exp-java-skipped-unit-tests-no-tests}{3}


==> tables/data-exp-skips-python.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-python-proj-initial}{31}
\DefMacro{exp-python-skipped}{2}
\DefMacro{exp-python-proj-can-run}{29}
\DefMacro{exp-python-skipped-import-error}{2}
\DefMacro{exp-python-skipped-unit-tests}{15}
\DefMacro{exp-python-proj-can-run-unit-tests}{14}
\DefMacro{exp-python-skipped-unit-tests-does-not-use-pytest}{5}
\DefMacro{exp-python-skipped-unit-tests-no-tests}{5}
\DefMacro{exp-python-skipped-unit-tests-too-many-test-failures}{5}


==> tables/data-exp-standalone-java.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-java-num-AVG-dup1-its}{1.30}
\DefMacro{exp-java-num-SUM-dup1-its}{65}
\DefMacro{exp-java-num-MAX-dup1-its}{5}
\DefMacro{exp-java-num-MIN-dup1-its}{1}
\DefMacro{exp-java-num-MEDIAN-dup1-its}{1.00}
\DefMacro{exp-java-num-STDEV-dup1-its}{0.67}
\DefMacro{exp-java-num-CNT-dup1-its}{50}
\DefMacro{exp-java-time-AVG-dup1-its}{0.46}
\DefMacro{exp-java-time-SUM-dup1-its}{23.08}
\DefMacro{exp-java-time-MAX-dup1-its}{0.51}
\DefMacro{exp-java-time-MIN-dup1-its}{0.44}
\DefMacro{exp-java-time-MEDIAN-dup1-its}{0.46}
\DefMacro{exp-java-time-STDEV-dup1-its}{0.01}
\DefMacro{exp-java-time-CNT-dup1-its}{50}
\DefMacro{exp-java-timept-AVG-dup1-its}{0.403}
\DefMacro{exp-java-timept-SUM-dup1-its}{20.175}
\DefMacro{exp-java-timept-MAX-dup1-its}{0.514}
\DefMacro{exp-java-timept-MIN-dup1-its}{0.092}
\DefMacro{exp-java-timept-MEDIAN-dup1-its}{0.454}
\DefMacro{exp-java-timept-STDEV-dup1-its}{0.106}
\DefMacro{exp-java-timept-CNT-dup1-its}{50}
\DefMacro{exp-java-timept-MACROAVG-dup1-its}{0.355}
\DefMacro{exp-java-num-AVG-dup10-its}{13.00}
\DefMacro{exp-java-num-SUM-dup10-its}{650}
\DefMacro{exp-java-num-MAX-dup10-its}{50}
\DefMacro{exp-java-num-MIN-dup10-its}{10}
\DefMacro{exp-java-num-MEDIAN-dup10-its}{10.00}
\DefMacro{exp-java-num-STDEV-dup10-its}{6.71}
\DefMacro{exp-java-num-CNT-dup10-its}{50}
\DefMacro{exp-java-time-AVG-dup10-its}{0.50}
\DefMacro{exp-java-time-SUM-dup10-its}{24.92}
\DefMacro{exp-java-time-MAX-dup10-its}{0.64}
\DefMacro{exp-java-time-MIN-dup10-its}{0.47}
\DefMacro{exp-java-time-MEDIAN-dup10-its}{0.49}
\DefMacro{exp-java-time-STDEV-dup10-its}{0.03}
\DefMacro{exp-java-time-CNT-dup10-its}{50}
\DefMacro{exp-java-timept-AVG-dup10-its}{0.043}
\DefMacro{exp-java-timept-SUM-dup10-its}{2.172}
\DefMacro{exp-java-timept-MAX-dup10-its}{0.064}
\DefMacro{exp-java-timept-MIN-dup10-its}{0.011}
\DefMacro{exp-java-timept-MEDIAN-dup10-its}{0.048}
\DefMacro{exp-java-timept-STDEV-dup10-its}{0.011}
\DefMacro{exp-java-timept-CNT-dup10-its}{50}
\DefMacro{exp-java-timept-MACROAVG-dup10-its}{0.038}
\DefMacro{exp-java-num-AVG-dup100-its}{130.00}
\DefMacro{exp-java-num-SUM-dup100-its}{6,500}
\DefMacro{exp-java-num-MAX-dup100-its}{500}
\DefMacro{exp-java-num-MIN-dup100-its}{100}
\DefMacro{exp-java-num-MEDIAN-dup100-its}{100.00}
\DefMacro{exp-java-num-STDEV-dup100-its}{67.08}
\DefMacro{exp-java-num-CNT-dup100-its}{50}
\DefMacro{exp-java-time-AVG-dup100-its}{0.68}
\DefMacro{exp-java-time-SUM-dup100-its}{34.21}
\DefMacro{exp-java-time-MAX-dup100-its}{1.03}
\DefMacro{exp-java-time-MIN-dup100-its}{0.58}
\DefMacro{exp-java-time-MEDIAN-dup100-its}{0.67}
\DefMacro{exp-java-time-STDEV-dup100-its}{0.08}
\DefMacro{exp-java-time-CNT-dup100-its}{50}
\DefMacro{exp-java-timept-AVG-dup100-its}{0.006}
\DefMacro{exp-java-timept-SUM-dup100-its}{0.296}
\DefMacro{exp-java-timept-MAX-dup100-its}{0.010}
\DefMacro{exp-java-timept-MIN-dup100-its}{0.002}
\DefMacro{exp-java-timept-MEDIAN-dup100-its}{0.006}
\DefMacro{exp-java-timept-STDEV-dup100-its}{0.002}
\DefMacro{exp-java-timept-CNT-dup100-its}{50}
\DefMacro{exp-java-timept-MACROAVG-dup100-its}{0.005}
\DefMacro{exp-java-num-AVG-dup1000-its}{1,300.00}
\DefMacro{exp-java-num-SUM-dup1000-its}{65,000}
\DefMacro{exp-java-num-MAX-dup1000-its}{5,000}
\DefMacro{exp-java-num-MIN-dup1000-its}{1,000}
\DefMacro{exp-java-num-MEDIAN-dup1000-its}{1,000.00}
\DefMacro{exp-java-num-STDEV-dup1000-its}{670.82}
\DefMacro{exp-java-num-CNT-dup1000-its}{50}
\DefMacro{exp-java-time-AVG-dup1000-its}{1.36}
\DefMacro{exp-java-time-SUM-dup1000-its}{67.87}
\DefMacro{exp-java-time-MAX-dup1000-its}{3.03}
\DefMacro{exp-java-time-MIN-dup1000-its}{0.97}
\DefMacro{exp-java-time-MEDIAN-dup1000-its}{1.25}
\DefMacro{exp-java-time-STDEV-dup1000-its}{0.40}
\DefMacro{exp-java-time-CNT-dup1000-its}{50}
\DefMacro{exp-java-timept-AVG-dup1000-its}{0.001}
\DefMacro{exp-java-timept-SUM-dup1000-its}{0.057}
\DefMacro{exp-java-timept-MAX-dup1000-its}{0.003}
\DefMacro{exp-java-timept-MIN-dup1000-its}{0.001}
\DefMacro{exp-java-timept-MEDIAN-dup1000-its}{0.001}
\DefMacro{exp-java-timept-STDEV-dup1000-its}{0.000}
\DefMacro{exp-java-timept-CNT-dup1000-its}{50}
\DefMacro{exp-java-timept-MACROAVG-dup1000-its}{0.001}


==> tables/data-exp-standalone-python.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{exp-python-num-AVG-dup1-its}{1.74}
\DefMacro{exp-python-num-SUM-dup1-its}{87}
\DefMacro{exp-python-num-MAX-dup1-its}{4}
\DefMacro{exp-python-num-MIN-dup1-its}{1}
\DefMacro{exp-python-num-MEDIAN-dup1-its}{1.00}
\DefMacro{exp-python-num-STDEV-dup1-its}{0.91}
\DefMacro{exp-python-num-CNT-dup1-its}{50}
\DefMacro{exp-python-time-AVG-dup1-its}{0.16}
\DefMacro{exp-python-time-SUM-dup1-its}{8.21}
\DefMacro{exp-python-time-MAX-dup1-its}{0.32}
\DefMacro{exp-python-time-MIN-dup1-its}{0.16}
\DefMacro{exp-python-time-MEDIAN-dup1-its}{0.16}
\DefMacro{exp-python-time-STDEV-dup1-its}{0.02}
\DefMacro{exp-python-time-CNT-dup1-its}{50}
\DefMacro{exp-python-timept-AVG-dup1-its}{0.119}
\DefMacro{exp-python-timept-SUM-dup1-its}{5.955}
\DefMacro{exp-python-timept-MAX-dup1-its}{0.324}
\DefMacro{exp-python-timept-MIN-dup1-its}{0.040}
\DefMacro{exp-python-timept-MEDIAN-dup1-its}{0.159}
\DefMacro{exp-python-timept-STDEV-dup1-its}{0.055}
\DefMacro{exp-python-timept-CNT-dup1-its}{50}
\DefMacro{exp-python-timept-MACROAVG-dup1-its}{0.094}
\DefMacro{exp-python-num-AVG-dup10-its}{17.40}
\DefMacro{exp-python-num-SUM-dup10-its}{870}
\DefMacro{exp-python-num-MAX-dup10-its}{40}
\DefMacro{exp-python-num-MIN-dup10-its}{10}
\DefMacro{exp-python-num-MEDIAN-dup10-its}{10.00}
\DefMacro{exp-python-num-STDEV-dup10-its}{9.12}
\DefMacro{exp-python-num-CNT-dup10-its}{50}
\DefMacro{exp-python-time-AVG-dup10-its}{0.18}
\DefMacro{exp-python-time-SUM-dup10-its}{8.84}
\DefMacro{exp-python-time-MAX-dup10-its}{0.34}
\DefMacro{exp-python-time-MIN-dup10-its}{0.17}
\DefMacro{exp-python-time-MEDIAN-dup10-its}{0.17}
\DefMacro{exp-python-time-STDEV-dup10-its}{0.03}
\DefMacro{exp-python-time-CNT-dup10-its}{50}
\DefMacro{exp-python-timept-AVG-dup10-its}{0.013}
\DefMacro{exp-python-timept-SUM-dup10-its}{0.634}
\DefMacro{exp-python-timept-MAX-dup10-its}{0.034}
\DefMacro{exp-python-timept-MIN-dup10-its}{0.005}
\DefMacro{exp-python-timept-MEDIAN-dup10-its}{0.017}
\DefMacro{exp-python-timept-STDEV-dup10-its}{0.006}
\DefMacro{exp-python-timept-CNT-dup10-its}{50}
\DefMacro{exp-python-timept-MACROAVG-dup10-its}{0.010}
\DefMacro{exp-python-num-AVG-dup100-its}{174.00}
\DefMacro{exp-python-num-SUM-dup100-its}{8,700}
\DefMacro{exp-python-num-MAX-dup100-its}{400}
\DefMacro{exp-python-num-MIN-dup100-its}{100}
\DefMacro{exp-python-num-MEDIAN-dup100-its}{100.00}
\DefMacro{exp-python-num-STDEV-dup100-its}{91.24}
\DefMacro{exp-python-num-CNT-dup100-its}{50}
\DefMacro{exp-python-time-AVG-dup100-its}{0.30}
\DefMacro{exp-python-time-SUM-dup100-its}{15.21}
\DefMacro{exp-python-time-MAX-dup100-its}{0.53}
\DefMacro{exp-python-time-MIN-dup100-its}{0.23}
\DefMacro{exp-python-time-MEDIAN-dup100-its}{0.28}
\DefMacro{exp-python-time-STDEV-dup100-its}{0.08}
\DefMacro{exp-python-time-CNT-dup100-its}{50}
\DefMacro{exp-python-timept-AVG-dup100-its}{0.002}
\DefMacro{exp-python-timept-SUM-dup100-its}{0.101}
\DefMacro{exp-python-timept-MAX-dup100-its}{0.005}
\DefMacro{exp-python-timept-MIN-dup100-its}{0.001}
\DefMacro{exp-python-timept-MEDIAN-dup100-its}{0.002}
\DefMacro{exp-python-timept-STDEV-dup100-its}{0.001}
\DefMacro{exp-python-timept-CNT-dup100-its}{50}
\DefMacro{exp-python-timept-MACROAVG-dup100-its}{0.002}
\DefMacro{exp-python-num-AVG-dup1000-its}{1,740.00}
\DefMacro{exp-python-num-SUM-dup1000-its}{87,000}
\DefMacro{exp-python-num-MAX-dup1000-its}{4,000}
\DefMacro{exp-python-num-MIN-dup1000-its}{1,000}
\DefMacro{exp-python-num-MEDIAN-dup1000-its}{1,000.00}
\DefMacro{exp-python-num-STDEV-dup1000-its}{912.36}
\DefMacro{exp-python-num-CNT-dup1000-its}{50}
\DefMacro{exp-python-time-AVG-dup1000-its}{2.40}
\DefMacro{exp-python-time-SUM-dup1000-its}{120.17}
\DefMacro{exp-python-time-MAX-dup1000-its}{6.13}
\DefMacro{exp-python-time-MIN-dup1000-its}{1.14}
\DefMacro{exp-python-time-MEDIAN-dup1000-its}{2.12}
\DefMacro{exp-python-time-STDEV-dup1000-its}{1.24}
\DefMacro{exp-python-time-CNT-dup1000-its}{50}
\DefMacro{exp-python-timept-AVG-dup1000-its}{0.001}
\DefMacro{exp-python-timept-SUM-dup1000-its}{0.071}
\DefMacro{exp-python-timept-MAX-dup1000-its}{0.003}
\DefMacro{exp-python-timept-MIN-dup1000-its}{0.001}
\DefMacro{exp-python-timept-MEDIAN-dup1000-its}{0.001}
\DefMacro{exp-python-timept-STDEV-dup1000-its}{0.000}
\DefMacro{exp-python-timept-CNT-dup1000-its}{50}
\DefMacro{exp-python-timept-MACROAVG-dup1000-its}{0.001}


==> tables/data-java-inline-tests-category.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{NumJavaRegexTestedStmts}{17}
\DefMacro{NumJavaRegexInlineTests}{17}
\DefMacro{NumJavaRegexProjs}{15}
\DefMacro{NumJavaRegexFiles}{17}
\DefMacro{NumJavaStringTestedStmts}{20}
\DefMacro{NumJavaStringInlineTests}{20}
\DefMacro{NumJavaStringProjs}{15}
\DefMacro{NumJavaStringFiles}{15}
\DefMacro{NumJavaBitTestedStmts}{25}
\DefMacro{NumJavaBitInlineTests}{26}
\DefMacro{NumJavaBitProjs}{16}
\DefMacro{NumJavaBitFiles}{16}
\DefMacro{NumJavaStreamTestedStmts}{2}
\DefMacro{NumJavaStreamInlineTests}{2}
\DefMacro{NumJavaStreamProjs}{2}
\DefMacro{NumJavaStreamFiles}{2}
\DefMacro{NumJavaTestedStmts}{64}
\DefMacro{NumJavaInlineTests}{65}
\DefMacro{NumJavaProjs}{37}
\DefMacro{NumJavaFiles}{50}


==> tables/data-python-inline-tests-category.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{NumPythonRegexTestedStmts}{19}
\DefMacro{NumPythonRegexInlineTests}{22}
\DefMacro{NumPythonRegexProjs}{15}
\DefMacro{NumPythonRegexFiles}{17}
\DefMacro{NumPythonStringTestedStmts}{30}
\DefMacro{NumPythonStringInlineTests}{32}
\DefMacro{NumPythonStringProjs}{13}
\DefMacro{NumPythonStringFiles}{14}
\DefMacro{NumPythonBitTestedStmts}{26}
\DefMacro{NumPythonBitInlineTests}{27}
\DefMacro{NumPythonBitProjs}{15}
\DefMacro{NumPythonBitFiles}{15}
\DefMacro{NumPythonCollectionTestedStmts}{5}
\DefMacro{NumPythonCollectionInlineTests}{6}
\DefMacro{NumPythonCollectionProjs}{4}
\DefMacro{NumPythonCollectionFiles}{4}
\DefMacro{NumPythonProjs}{31}
\DefMacro{NumPythonFiles}{50}
\DefMacro{NumPythonInlineTests}{87}
\DefMacro{NumPythonTestedStmts}{80}


==> tables/data-userstudy-res.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{AVG_difficulty_of_learning}{4.2}
\DefMacro{SUM_difficulty_of_learning}{38.0}
\DefMacro{MAX_difficulty_of_learning}{5.0}
\DefMacro{MIN_difficulty_of_learning}{3.0}
\DefMacro{MEDIAN_difficulty_of_learning}{4.0}
\DefMacro{STDEV_difficulty_of_learning}{0.8}
\DefMacro{CNT_difficulty_of_learning}{9.0}
\DefMacro{AVG_difficulty_of_using}{4.1}
\DefMacro{SUM_difficulty_of_using}{37.0}
\DefMacro{MAX_difficulty_of_using}{5.0}
\DefMacro{MIN_difficulty_of_using}{3.0}
\DefMacro{MEDIAN_difficulty_of_using}{4.0}
\DefMacro{STDEV_difficulty_of_using}{0.6}
\DefMacro{CNT_difficulty_of_using}{9.0}
\DefMacro{AVG_years_of_programming}{6.1}
\DefMacro{SUM_years_of_programming}{55.0}
\DefMacro{MAX_years_of_programming}{12.0}
\DefMacro{MIN_years_of_programming}{3.0}
\DefMacro{MEDIAN_years_of_programming}{6.0}
\DefMacro{STDEV_years_of_programming}{2.6}
\DefMacro{CNT_years_of_programming}{9.0}
\DefMacro{AVG_python_expertise}{3.4}
\DefMacro{SUM_python_expertise}{30.5}
\DefMacro{MAX_python_expertise}{4.0}
\DefMacro{MIN_python_expertise}{3.0}
\DefMacro{MEDIAN_python_expertise}{3.0}
\DefMacro{STDEV_python_expertise}{0.5}
\DefMacro{CNT_python_expertise}{9.0}
\DefMacro{AVG_task_1_time_per_test}{2.8}
\DefMacro{SUM_task_1_time_per_test}{24.8}
\DefMacro{MAX_task_1_time_per_test}{9.0}
\DefMacro{MIN_task_1_time_per_test}{0.5}
\DefMacro{MEDIAN_task_1_time_per_test}{2.0}
\DefMacro{STDEV_task_1_time_per_test}{2.6}
\DefMacro{CNT_task_1_time_per_test}{9.0}
\DefMacro{AVG_task_1_understanding_time}{4.0}
\DefMacro{SUM_task_1_understanding_time}{36.0}
\DefMacro{MAX_task_1_understanding_time}{8.0}
\DefMacro{MIN_task_1_understanding_time}{1.0}
\DefMacro{MEDIAN_task_1_understanding_time}{4.0}
\DefMacro{STDEV_task_1_understanding_time}{2.7}
\DefMacro{CNT_task_1_understanding_time}{9.0}
\DefMacro{AVG_task_1_writing_time}{3.7}
\DefMacro{SUM_task_1_writing_time}{33.0}
\DefMacro{MAX_task_1_writing_time}{9.0}
\DefMacro{MIN_task_1_writing_time}{1.0}
\DefMacro{MEDIAN_task_1_writing_time}{3.0}
\DefMacro{STDEV_task_1_writing_time}{2.6}
\DefMacro{CNT_task_1_writing_time}{9.0}
\DefMacro{AVG_task_1_num_tests}{1.7}
\DefMacro{SUM_task_1_num_tests}{15.0}
\DefMacro{MAX_task_1_num_tests}{3.0}
\DefMacro{MIN_task_1_num_tests}{1.0}
\DefMacro{MEDIAN_task_1_num_tests}{1.0}
\DefMacro{STDEV_task_1_num_tests}{0.8}
\DefMacro{CNT_task_1_num_tests}{9.0}
\DefMacro{AVG_task_1_num_passed_tests}{1.7}
\DefMacro{SUM_task_1_num_passed_tests}{15.0}
\DefMacro{MAX_task_1_num_passed_tests}{3.0}
\DefMacro{MIN_task_1_num_passed_tests}{1.0}
\DefMacro{MEDIAN_task_1_num_passed_tests}{1.0}
\DefMacro{STDEV_task_1_num_passed_tests}{0.8}
\DefMacro{CNT_task_1_num_passed_tests}{9.0}
\DefMacro{AVG_task_2_time_per_test}{2.5}
\DefMacro{SUM_task_2_time_per_test}{22.2}
\DefMacro{MAX_task_2_time_per_test}{5.0}
\DefMacro{MIN_task_2_time_per_test}{1.5}
\DefMacro{MEDIAN_task_2_time_per_test}{2.0}
\DefMacro{STDEV_task_2_time_per_test}{1.0}
\DefMacro{CNT_task_2_time_per_test}{9.0}
\DefMacro{AVG_task_2_understanding_time}{1.6}
\DefMacro{SUM_task_2_understanding_time}{14.0}
\DefMacro{MAX_task_2_understanding_time}{3.0}
\DefMacro{MIN_task_2_understanding_time}{1.0}
\DefMacro{MEDIAN_task_2_understanding_time}{1.0}
\DefMacro{STDEV_task_2_understanding_time}{0.7}
\DefMacro{CNT_task_2_understanding_time}{9.0}
\DefMacro{AVG_task_2_writing_time}{3.4}
\DefMacro{SUM_task_2_writing_time}{31.0}
\DefMacro{MAX_task_2_writing_time}{5.0}
\DefMacro{MIN_task_2_writing_time}{2.0}
\DefMacro{MEDIAN_task_2_writing_time}{3.0}
\DefMacro{STDEV_task_2_writing_time}{1.1}
\DefMacro{CNT_task_2_writing_time}{9.0}
\DefMacro{AVG_task_2_num_tests}{1.6}
\DefMacro{SUM_task_2_num_tests}{14.0}
\DefMacro{MAX_task_2_num_tests}{3.0}
\DefMacro{MIN_task_2_num_tests}{1.0}
\DefMacro{MEDIAN_task_2_num_tests}{1.0}
\DefMacro{STDEV_task_2_num_tests}{0.7}
\DefMacro{CNT_task_2_num_tests}{9.0}
\DefMacro{AVG_task_2_num_passed_tests}{1.6}
\DefMacro{SUM_task_2_num_passed_tests}{14.0}
\DefMacro{MAX_task_2_num_passed_tests}{3.0}
\DefMacro{MIN_task_2_num_passed_tests}{1.0}
\DefMacro{MEDIAN_task_2_num_passed_tests}{1.0}
\DefMacro{STDEV_task_2_num_passed_tests}{0.7}
\DefMacro{CNT_task_2_num_passed_tests}{9.0}
\DefMacro{AVG_task_3_time_per_test}{3.0}
\DefMacro{SUM_task_3_time_per_test}{27.0}
\DefMacro{MAX_task_3_time_per_test}{9.0}
\DefMacro{MIN_task_3_time_per_test}{1.0}
\DefMacro{MEDIAN_task_3_time_per_test}{2.0}
\DefMacro{STDEV_task_3_time_per_test}{2.4}
\DefMacro{CNT_task_3_time_per_test}{9.0}
\DefMacro{AVG_task_3_understanding_time}{2.2}
\DefMacro{SUM_task_3_understanding_time}{20.0}
\DefMacro{MAX_task_3_understanding_time}{5.0}
\DefMacro{MIN_task_3_understanding_time}{0.0}
\DefMacro{MEDIAN_task_3_understanding_time}{2.0}
\DefMacro{STDEV_task_3_understanding_time}{1.5}
\DefMacro{CNT_task_3_understanding_time}{9.0}
\DefMacro{AVG_task_3_writing_time}{4.1}
\DefMacro{SUM_task_3_writing_time}{37.0}
\DefMacro{MAX_task_3_writing_time}{9.0}
\DefMacro{MIN_task_3_writing_time}{2.0}
\DefMacro{MEDIAN_task_3_writing_time}{4.0}
\DefMacro{STDEV_task_3_writing_time}{2.1}
\DefMacro{CNT_task_3_writing_time}{9.0}
\DefMacro{AVG_task_3_num_tests}{1.7}
\DefMacro{SUM_task_3_num_tests}{15.0}
\DefMacro{MAX_task_3_num_tests}{2.0}
\DefMacro{MIN_task_3_num_tests}{1.0}
\DefMacro{MEDIAN_task_3_num_tests}{2.0}
\DefMacro{STDEV_task_3_num_tests}{0.5}
\DefMacro{CNT_task_3_num_tests}{9.0}
\DefMacro{AVG_task_3_num_passed_tests}{1.7}
\DefMacro{SUM_task_3_num_passed_tests}{15.0}
\DefMacro{MAX_task_3_num_passed_tests}{2.0}
\DefMacro{MIN_task_3_num_passed_tests}{1.0}
\DefMacro{MEDIAN_task_3_num_passed_tests}{2.0}
\DefMacro{STDEV_task_3_num_passed_tests}{0.5}
\DefMacro{CNT_task_3_num_passed_tests}{9.0}
\DefMacro{AVG_task_4_time_per_test}{1.9}
\DefMacro{SUM_task_4_time_per_test}{17.3}
\DefMacro{MAX_task_4_time_per_test}{5.0}
\DefMacro{MIN_task_4_time_per_test}{0.3}
\DefMacro{MEDIAN_task_4_time_per_test}{1.0}
\DefMacro{STDEV_task_4_time_per_test}{1.7}
\DefMacro{CNT_task_4_time_per_test}{9.0}
\DefMacro{AVG_task_4_understanding_time}{3.3}
\DefMacro{SUM_task_4_understanding_time}{30.0}
\DefMacro{MAX_task_4_understanding_time}{8.0}
\DefMacro{MIN_task_4_understanding_time}{1.0}
\DefMacro{MEDIAN_task_4_understanding_time}{3.0}
\DefMacro{STDEV_task_4_understanding_time}{2.2}
\DefMacro{CNT_task_4_understanding_time}{9.0}
\DefMacro{AVG_task_4_writing_time}{2.8}
\DefMacro{SUM_task_4_writing_time}{25.0}
\DefMacro{MAX_task_4_writing_time}{6.0}
\DefMacro{MIN_task_4_writing_time}{1.0}
\DefMacro{MEDIAN_task_4_writing_time}{2.0}
\DefMacro{STDEV_task_4_writing_time}{1.9}
\DefMacro{CNT_task_4_writing_time}{9.0}
\DefMacro{AVG_task_4_num_tests}{1.8}
\DefMacro{SUM_task_4_num_tests}{16.0}
\DefMacro{MAX_task_4_num_tests}{3.0}
\DefMacro{MIN_task_4_num_tests}{1.0}
\DefMacro{MEDIAN_task_4_num_tests}{2.0}
\DefMacro{STDEV_task_4_num_tests}{0.8}
\DefMacro{CNT_task_4_num_tests}{9.0}
\DefMacro{AVG_task_4_num_passed_tests}{1.8}
\DefMacro{SUM_task_4_num_passed_tests}{16.0}
\DefMacro{MAX_task_4_num_passed_tests}{3.0}
\DefMacro{MIN_task_4_num_passed_tests}{1.0}
\DefMacro{MEDIAN_task_4_num_passed_tests}{2.0}
\DefMacro{STDEV_task_4_num_passed_tests}{0.8}
\DefMacro{CNT_task_4_num_passed_tests}{9.0}
\DefMacro{AVG_time_per_test}{2.5}
\DefMacro{MEDIAN_time_per_test}{2.6}
\DefMacro{AVG_understanding_time}{2.8}
\DefMacro{MEDIAN_understanding_time}{2.8}
\DefMacro{AVG_writing_time}{3.5}
\DefMacro{MEDIAN_writing_time}{3.6}
\DefMacro{AVG_num_tests}{1.7}
\DefMacro{MEDIAN_num_tests}{1.7}
\DefMacro{task_1_benefit}{8}
\DefMacro{task_2_benefit}{8}
\DefMacro{task_3_benefit}{5}
\DefMacro{task_4_benefit}{9}
\DefMacro{task_1_correct_times}{9}
\DefMacro{task_2_correct_times}{9}
\DefMacro{task_3_correct_times}{9}
\DefMacro{task_4_correct_times}{9}
\DefMacro{NumUsers}{9}


==> tables/table-exp-integrated-dups-python-one-column.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline
\HeaderDup & \HeaderNumVanilla & \HeaderNumITOnly & \HeaderTimeVanilla & \HeaderTimeITEnabled & \HeaderOverheadITEnabled & \HeaderTimeITDisabled & \HeaderOverheadITDisabled \\
\hline
\UseMacro{dup-1}
 & \UseMacro{exp-python-num-vanilla-SUM-dup1}
 & \UseMacro{exp-python-num-inline-SUM-dup1}
 & \UseMacro{exp-python-time-vanilla-SUM-dup1}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup1}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1}
 & \UseMacro{exp-python-time-unit-SUM-dup1}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup1}
 \\
\UseMacro{dup-10}
 & \UseMacro{exp-python-num-vanilla-SUM-dup10}
 & \UseMacro{exp-python-num-inline-SUM-dup10}
 & \UseMacro{exp-python-time-vanilla-SUM-dup10}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup10}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup10}
 & \UseMacro{exp-python-time-unit-SUM-dup10}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup10}
 \\
\UseMacro{dup-100}
 & \UseMacro{exp-python-num-vanilla-SUM-dup100}
 & \UseMacro{exp-python-num-inline-SUM-dup100}
 & \UseMacro{exp-python-time-vanilla-SUM-dup100}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup100}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup100}
 & \UseMacro{exp-python-time-unit-SUM-dup100}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup100}
 \\
\UseMacro{dup-1000}
 & \UseMacro{exp-python-num-vanilla-SUM-dup1000}
 & \UseMacro{exp-python-num-inline-SUM-dup1000}
 & \UseMacro{exp-python-time-vanilla-SUM-dup1000}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup1000}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1000}
 & \UseMacro{exp-python-time-unit-SUM-dup1000}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup1000}
 \\
\hline
\end{tabular}


==> tables/table-exp-integrated-dups-python.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{|l|r|r||r|r||r|r|r||r|r|r|}
\hline
\HeaderDup & \HeaderNumVanilla & \HeaderNumITOnly & \HeaderTimeVanilla & \HeaderTimePerTestVanilla & \HeaderTimeITEnabled & \HeaderTimePerTestITEnabled & \HeaderOverheadITEnabled & \HeaderTimeITDisabled & \HeaderTimePerTestITDisabled & \HeaderOverheadITDisabled \\
\hline
\UseMacro{dup-1}
 & \UseMacro{exp-python-num-vanilla-SUM-dup1}
 & \UseMacro{exp-python-num-inline-SUM-dup1}
 & \UseMacro{exp-python-time-vanilla-SUM-dup1}
 & \UseMacro{exp-python-timept-vanilla-MACROAVG-dup1}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup1}
 & \UseMacro{exp-python-timept-unit-and-inline-MACROAVG-dup1}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1}
 & \UseMacro{exp-python-time-unit-SUM-dup1}
 & \UseMacro{exp-python-timept-unit-MACROAVG-dup1}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup1}
 \\
\UseMacro{dup-10}
 & \UseMacro{exp-python-num-vanilla-SUM-dup10}
 & \UseMacro{exp-python-num-inline-SUM-dup10}
 & \UseMacro{exp-python-time-vanilla-SUM-dup10}
 & \UseMacro{exp-python-timept-vanilla-MACROAVG-dup10}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup10}
 & \UseMacro{exp-python-timept-unit-and-inline-MACROAVG-dup10}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup10}
 & \UseMacro{exp-python-time-unit-SUM-dup10}
 & \UseMacro{exp-python-timept-unit-MACROAVG-dup10}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup10}
 \\
\UseMacro{dup-100}
 & \UseMacro{exp-python-num-vanilla-SUM-dup100}
 & \UseMacro{exp-python-num-inline-SUM-dup100}
 & \UseMacro{exp-python-time-vanilla-SUM-dup100}
 & \UseMacro{exp-python-timept-vanilla-MACROAVG-dup100}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup100}
 & \UseMacro{exp-python-timept-unit-and-inline-MACROAVG-dup100}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup100}
 & \UseMacro{exp-python-time-unit-SUM-dup100}
 & \UseMacro{exp-python-timept-unit-MACROAVG-dup100}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup100}
 \\
\UseMacro{dup-1000}
 & \UseMacro{exp-python-num-vanilla-SUM-dup1000}
 & \UseMacro{exp-python-num-inline-SUM-dup1000}
 & \UseMacro{exp-python-time-vanilla-SUM-dup1000}
 & \UseMacro{exp-python-timept-vanilla-MACROAVG-dup1000}
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup1000}
 & \UseMacro{exp-python-timept-unit-and-inline-MACROAVG-dup1000}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1000}
 & \UseMacro{exp-python-time-unit-SUM-dup1000}
 & \UseMacro{exp-python-timept-unit-MACROAVG-dup1000}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup1000}
 \\
\hline
\end{tabular}


==> tables/table-exp-integrated-python.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{|l|r|r||r|r||r|r|r||r|r|r|}
\hline
\HeaderProj & \HeaderNumVanilla & \HeaderNumITOnly & \HeaderTimeVanilla & \HeaderTimePerTestVanilla & \HeaderTimeITEnabled & \HeaderTimePerTestITEnabled & \HeaderOverheadITEnabled & \HeaderTimeITDisabled & \HeaderTimePerTestITDisabled & \HeaderOverheadITDisabled \\
\hline
\UseMacro{proj-RaRe-Technologies_gensim}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-num-vanilla-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-num-inline-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-time-vanilla-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-timept-vanilla-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-time-unit-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-timept-unit-dup1}
 & \UseMacro{exp-python-RaRe-Technologies_gensim-overhead-unit-dup1}
 \\
\UseMacro{proj-Textualize_rich}
 & \UseMacro{exp-python-Textualize_rich-num-vanilla-dup1}
 & \UseMacro{exp-python-Textualize_rich-num-inline-dup1}
 & \UseMacro{exp-python-Textualize_rich-time-vanilla-dup1}
 & \UseMacro{exp-python-Textualize_rich-timept-vanilla-dup1}
 & \UseMacro{exp-python-Textualize_rich-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-Textualize_rich-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-Textualize_rich-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-Textualize_rich-time-unit-dup1}
 & \UseMacro{exp-python-Textualize_rich-timept-unit-dup1}
 & \UseMacro{exp-python-Textualize_rich-overhead-unit-dup1}
 \\
\UseMacro{proj-bokeh_bokeh}
 & \UseMacro{exp-python-bokeh_bokeh-num-vanilla-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-num-inline-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-time-vanilla-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-timept-vanilla-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-time-unit-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-timept-unit-dup1}
 & \UseMacro{exp-python-bokeh_bokeh-overhead-unit-dup1}
 \\
\UseMacro{proj-chubin_cheat.sh}
 & \UseMacro{exp-python-chubin_cheat.sh-num-vanilla-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-num-inline-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-time-vanilla-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-timept-vanilla-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-time-unit-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-timept-unit-dup1}
 & \UseMacro{exp-python-chubin_cheat.sh-overhead-unit-dup1}
 \\
\UseMacro{proj-davidsandberg_facenet}
 & \UseMacro{exp-python-davidsandberg_facenet-num-vanilla-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-num-inline-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-time-vanilla-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-timept-vanilla-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-time-unit-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-timept-unit-dup1}
 & \UseMacro{exp-python-davidsandberg_facenet-overhead-unit-dup1}
 \\
\UseMacro{proj-geekcomputers_Python}
 & \UseMacro{exp-python-geekcomputers_Python-num-vanilla-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-num-inline-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-time-vanilla-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-timept-vanilla-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-time-unit-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-timept-unit-dup1}
 & \UseMacro{exp-python-geekcomputers_Python-overhead-unit-dup1}
 \\
\UseMacro{proj-google-research_bert}
 & \UseMacro{exp-python-google-research_bert-num-vanilla-dup1}
 & \UseMacro{exp-python-google-research_bert-num-inline-dup1}
 & \UseMacro{exp-python-google-research_bert-time-vanilla-dup1}
 & \UseMacro{exp-python-google-research_bert-timept-vanilla-dup1}
 & \UseMacro{exp-python-google-research_bert-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-google-research_bert-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-google-research_bert-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-google-research_bert-time-unit-dup1}
 & \UseMacro{exp-python-google-research_bert-timept-unit-dup1}
 & \UseMacro{exp-python-google-research_bert-overhead-unit-dup1}
 \\
\UseMacro{proj-joke2k_faker}
 & \UseMacro{exp-python-joke2k_faker-num-vanilla-dup1}
 & \UseMacro{exp-python-joke2k_faker-num-inline-dup1}
 & \UseMacro{exp-python-joke2k_faker-time-vanilla-dup1}
 & \UseMacro{exp-python-joke2k_faker-timept-vanilla-dup1}
 & \UseMacro{exp-python-joke2k_faker-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-joke2k_faker-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-joke2k_faker-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-joke2k_faker-time-unit-dup1}
 & \UseMacro{exp-python-joke2k_faker-timept-unit-dup1}
 & \UseMacro{exp-python-joke2k_faker-overhead-unit-dup1}
 \\
\UseMacro{proj-mitmproxy_mitmproxy}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-num-vanilla-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-num-inline-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-time-vanilla-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-timept-vanilla-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-time-unit-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-timept-unit-dup1}
 & \UseMacro{exp-python-mitmproxy_mitmproxy-overhead-unit-dup1}
 \\
\UseMacro{proj-numpy_numpy}
 & \UseMacro{exp-python-numpy_numpy-num-vanilla-dup1}
 & \UseMacro{exp-python-numpy_numpy-num-inline-dup1}
 & \UseMacro{exp-python-numpy_numpy-time-vanilla-dup1}
 & \UseMacro{exp-python-numpy_numpy-timept-vanilla-dup1}
 & \UseMacro{exp-python-numpy_numpy-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-numpy_numpy-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-numpy_numpy-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-numpy_numpy-time-unit-dup1}
 & \UseMacro{exp-python-numpy_numpy-timept-unit-dup1}
 & \UseMacro{exp-python-numpy_numpy-overhead-unit-dup1}
 \\
\UseMacro{proj-pandas-dev_pandas}
 & \UseMacro{exp-python-pandas-dev_pandas-num-vanilla-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-num-inline-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-time-vanilla-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-timept-vanilla-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-time-unit-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-timept-unit-dup1}
 & \UseMacro{exp-python-pandas-dev_pandas-overhead-unit-dup1}
 \\
\UseMacro{proj-psf_black}
 & \UseMacro{exp-python-psf_black-num-vanilla-dup1}
 & \UseMacro{exp-python-psf_black-num-inline-dup1}
 & \UseMacro{exp-python-psf_black-time-vanilla-dup1}
 & \UseMacro{exp-python-psf_black-timept-vanilla-dup1}
 & \UseMacro{exp-python-psf_black-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-psf_black-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-psf_black-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-psf_black-time-unit-dup1}
 & \UseMacro{exp-python-psf_black-timept-unit-dup1}
 & \UseMacro{exp-python-psf_black-overhead-unit-dup1}
 \\
\UseMacro{proj-pypa_pipenv}
 & \UseMacro{exp-python-pypa_pipenv-num-vanilla-dup1}
 & \UseMacro{exp-python-pypa_pipenv-num-inline-dup1}
 & \UseMacro{exp-python-pypa_pipenv-time-vanilla-dup1}
 & \UseMacro{exp-python-pypa_pipenv-timept-vanilla-dup1}
 & \UseMacro{exp-python-pypa_pipenv-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-pypa_pipenv-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-pypa_pipenv-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-pypa_pipenv-time-unit-dup1}
 & \UseMacro{exp-python-pypa_pipenv-timept-unit-dup1}
 & \UseMacro{exp-python-pypa_pipenv-overhead-unit-dup1}
 \\
\UseMacro{proj-scrapy_scrapy}
 & \UseMacro{exp-python-scrapy_scrapy-num-vanilla-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-num-inline-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-time-vanilla-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-timept-vanilla-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-time-unit-and-inline-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-timept-unit-and-inline-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-overhead-unit-and-inline-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-time-unit-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-timept-unit-dup1}
 & \UseMacro{exp-python-scrapy_scrapy-overhead-unit-dup1}
 \\
\hline
\HeaderAvg
 & \UseMacro{exp-python-num-vanilla-AVG-dup1}
 & \UseMacro{exp-python-num-inline-AVG-dup1}
 & \UseMacro{exp-python-time-vanilla-AVG-dup1}
 & \UseMacro{exp-python-timept-vanilla-MACROAVG-dup1}
 & \UseMacro{exp-python-time-unit-and-inline-AVG-dup1}
 & \UseMacro{exp-python-timept-unit-and-inline-MACROAVG-dup1}
 & \UseMacro{exp-python-overhead-unit-and-inline-MACROAVG-dup1}
 & \UseMacro{exp-python-time-unit-AVG-dup1}
 & \UseMacro{exp-python-timept-unit-MACROAVG-dup1}
 & \UseMacro{exp-python-overhead-unit-MACROAVG-dup1}
 \\
\HeaderSum
 & \UseMacro{exp-python-num-vanilla-SUM-dup1}
 & \UseMacro{exp-python-num-inline-SUM-dup1}
 & \UseMacro{exp-python-time-vanilla-SUM-dup1}
 & \HeaderNA
 & \UseMacro{exp-python-time-unit-and-inline-SUM-dup1}
 & \HeaderNA
 & \HeaderNA
 & \UseMacro{exp-python-time-unit-SUM-dup1}
 & \HeaderNA
 & \HeaderNA
 \\
\hline
\end{tabular}


==> tables/table-feature.tex <==
\begin{table*}[t!]
    \begin{center}
    % \vspace{-10px}    
    \caption{\CaptionITestFeature}
    % \vspace{-10px}
    % \scalebox{0.85}{
    \begin{tabular}{|L{0.1cm}|m{2cm}|m{5.8cm}|m{6.5cm}|}
        \hline
        & \textbf{Feature} & \textbf{Description} & \textbf{Example}\\
        \hline
        % \rowcolor{black!10}\multicolumn{2}{|l|}{Declaration}\\
        % \cline{1-2}
        \multirow[c]{7}{*}{\rotatebox{90}{Prototype}} & display name & Provide custom \inlinetest name & \UseMacro{itest-constructor-code}\Code{(test_name="check_match_name")...}\\
        \cline{2-4}
        & parameterization & Provide multiple inputs to an \inlinetest & \UseMacro{itest-constructor-code}(parameterized=True).given(name,["a:0","a:1:1"]) .check\_eq(m.group(1), ["a", "a:1"])\\
        \cline{2-4}
        & repetition & Specify number of times to run an \inlinetest & \UseMacro{itest-constructor-code}\Code{(repeated=2)...}\\
        \cline{2-4}
        & tags & Tag \inlinetests to aid filtering & \makecell[l]{\UseMacro{itest-constructor-code}\Code{(tag=["regex"])...}\\\texttt{\$ pytest \mbox{-}\mbox{-}inlinetest-group="tag-name"}}\\
        \cline{2-4}
        & disabling tests & Disable an \inlinetest & \UseMacro{itest-constructor-code}\Code{(disabled=True)...}\\
        \hline
        \multirow[c]{6}{*}{\rotatebox{90}{New}} & timeout & Fail if \inlinetest is still running after \CodeIn{n} seconds & \UseMacro{itest-constructor-code}\Code{(timeout=5)...}\\
        \cline{2-4}
        & assumptions & Execute \inlinetest only if an assumption holds & \UseMacro{itest-constructor-code}\Code{().assume(platform.system() == "Linux")...}\\
        \cline{2-4}
        & \inlinetests order & Prioritize \inlinetests & \texttt{\$ pytest \mbox{-}\mbox{-}inlinetest-order="tag-name"}\\
        \cline{2-4}
        & parallel runs & Run \inlinetests in parallel using \textit{pytest-xdist}~\cite{PytestXdist} & \texttt{\$ pytest -n auto}\\
        \cline{2-4}
        & new oracles & \makecell[l]{\Code{check_neq}, \Code{check_none}, \Code{check_not_none},\\ \Code{check_same}, \Code{check_not_same}} & \UseMacro{itest-constructor-code}\Code{().given(name, "a:a").check_none(m)}\\
        \hline
    \end{tabular}
    % }
    \end{center}
    \vspace{-15px}
\end{table*}


==> tables/table-userstudy-res.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
  \begin{center}
    \vspace{-10px}
\caption{\TitleUserStudyResults}
% \vspace{-10px}
\scalebox{0.8}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\HeaderTask & \multicolumn{2}{l|}{\HeaderUnderstandingTime} &  \multicolumn{2}{l|}{\HeaderWritingTime} &  \multicolumn{2}{l|}{\HeaderNumTests} &  \multicolumn{2}{l|}{\HeaderWritingTimePerTest} & \HeaderNumPassedTests & \HeaderBenefits \\
\cline{2-9}
 & \HeaderAvg & \HeaderMed & \HeaderAvg & \HeaderMed & \HeaderAvg & \HeaderMed & \HeaderAvg & \HeaderMed & & \\
\hline
1
 & \UseMacro{AVG_task_1_understanding_time}
 & \UseMacro{MEDIAN_task_1_understanding_time}
 & \UseMacro{AVG_task_1_writing_time}
 & \UseMacro{MEDIAN_task_1_writing_time}
 & \UseMacro{AVG_task_1_num_tests}
 & \UseMacro{MEDIAN_task_1_num_tests}
 & \UseMacro{AVG_task_1_time_per_test}
 & \UseMacro{MEDIAN_task_1_time_per_test}
 & \UseMacro{task_1_correct_times}/\UseMacro{NumUsers}
 & \UseMacro{task_1_benefit}/\UseMacro{NumUsers}
\\
\hline
2
 & \UseMacro{AVG_task_2_understanding_time}
 & \UseMacro{MEDIAN_task_2_understanding_time}
 & \UseMacro{AVG_task_2_writing_time}
 & \UseMacro{MEDIAN_task_2_writing_time}
 & \UseMacro{AVG_task_2_num_tests}
 & \UseMacro{MEDIAN_task_2_num_tests}
 & \UseMacro{AVG_task_2_time_per_test}
 & \UseMacro{MEDIAN_task_2_time_per_test}
 & \UseMacro{task_2_correct_times}/\UseMacro{NumUsers}
 & \UseMacro{task_2_benefit}/\UseMacro{NumUsers}
\\
\hline
3
 & \UseMacro{AVG_task_3_understanding_time}
 & \UseMacro{MEDIAN_task_3_understanding_time}
 & \UseMacro{AVG_task_3_writing_time}
 & \UseMacro{MEDIAN_task_3_writing_time}
 & \UseMacro{AVG_task_3_num_tests}
 & \UseMacro{MEDIAN_task_3_num_tests}
 & \UseMacro{AVG_task_3_time_per_test}
 & \UseMacro{MEDIAN_task_3_time_per_test}
 & \UseMacro{task_3_correct_times}/\UseMacro{NumUsers}
 & \UseMacro{task_3_benefit}/\UseMacro{NumUsers}
\\
\hline
4
 & \UseMacro{AVG_task_4_understanding_time}
 & \UseMacro{MEDIAN_task_4_understanding_time}
 & \UseMacro{AVG_task_4_writing_time}
 & \UseMacro{MEDIAN_task_4_writing_time}
 & \UseMacro{AVG_task_4_num_tests}
 & \UseMacro{MEDIAN_task_4_num_tests}
 & \UseMacro{AVG_task_4_time_per_test}
 & \UseMacro{MEDIAN_task_4_time_per_test}
 & \UseMacro{task_4_correct_times}/\UseMacro{NumUsers}
 & \UseMacro{task_4_benefit}/\UseMacro{NumUsers}
\\
\hline
\HeaderAvg
 & \UseMacro{AVG_understanding_time}
 & \UseMacro{MEDIAN_understanding_time}
 & \UseMacro{AVG_writing_time}
 & \UseMacro{MEDIAN_writing_time}
 & \UseMacro{AVG_num_tests}
 & \UseMacro{MEDIAN_num_tests}
 & \UseMacro{AVG_time_per_test}
 & \UseMacro{MEDIAN_time_per_test}
 & \HeaderNA
 & \HeaderNA
\\
\hline
\end{tabular}
}
\label{table:user-study-res}
\end{center}
\end{table}

